The Art of CPU-Pinning: Evaluating and Improving the Performance of Virtualization and Containerization Platforms

Cloud providers offer a variety of execution platforms in form of bare-metal, VM, and containers. However, due to the pros and cons of each execution platform, choosing the appropriate platform for a specific cloud-based application has become a challenge for solution architects. The possibility to combine these platforms (e.g. deploying containers within VMs) offers new capacities that makes the challenge even further complicated. However, there is a little study in the literature on the pros and cons of deploying different application types on various execution platforms. In particular, evaluation of diverse hardware configurations and different CPU provisioning methods, such as CPU pinning, have not been sufficiently studied in the literature. In this work, the performance overhead of container, VM, and bare-metal execution platforms are measured and analyzed for four categories of real-world applications, namely video processing, parallel processing (MPI), web processing, and No-SQL, respectively representing CPU intensive, parallel processing, and two IO intensive processes. Our analyses reveal a set of interesting and sometimes counterintuitive findings that can be used as best practices by the solution architects to efficiently deploy cloud-based applications. Here are some notable mentions: (A) Under specific circumstances, containers can impose a higher overhead than VMs; (B) Containers on top of VMs can mitigate the overhead of VMs for certain applications; (C) Containers with a large number of cores impose a lower overhead than those with a few cores.

==> Sources/contingencyrank.tex <==
\begin{table*}[tp]
	\caption{Ranked (R) List of Cyber-Physical Contingencies (MDP edges)}
	\label{tab:cp-contingencies}
	\centering
	\tiny
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} \\ \hline
		0 & $0,74$ & 1 & $0,1$ & 2 & $0,146$ & 3 & $74,125$ & 4 & $74,101$ & 5 & $74,2$ & 6 & $74,134$ & 7 & $74,142$ & 8 & $74,76$ & 9 & $1,2$\\ \hline
		10 & $1,73$ & 11 & $146,142$ & 12 & $146,73$ & 13 & $125,126$ & 14 & $101,123$ & 15 & $101,102$ & 16 & $101,111$ & 17 & $101,119$ & 18 & $101,28$ & 19 & $101,77$\\ \hline
		20 & $2,52$ & 21 & $2,28$ & 22 & $2,3$ & 23 & $2,61$ & 24 & $2,69$ & 25 & $134,139$ & 26 & $134,111$ & 27 & $134,61$ & 28 & $134,135$ & 29 & $134,141$\\ \hline
		30 & $142,145$ & 31 & $142,119$ & 32 & $142,69$ & 33 & $142,143$ & 34 & $142,141$ & 35 & $76,77$ & 36 & $73,69$ & 37 & $126,53$ & 38 & $126,127$ & 39 & $126,103$\\ \hline
		40 & $126,131$ & 41 & $126,133$ & 42 & $123,99$ & 43 & $123,124$ & 44 & $123,118$ & 45 & $123,122$ & 46 & $123,50$ & 47 & $102,103$ & 48 & $111,118$ & 49 & $111,112$\\ \hline
		50 & $111,116$ & 51 & $111,38$ & 52 & $111,87$ & 53 & $119,122$ & 54 & $119,120$ & 55 & $119,46$ & 56 & $119,116$ & 57 & $119,95$ & 58 & $28,50$ & 59 & $28,29$\\ \hline
		60 & $28,38$ & 61 & $28,46$ & 62 & $28,4$ & 63 & $77,99$ & 64 & $77,78$ & 65 & $77,95$ & 66 & $77,4$ & 67 & $77,87$ & 68 & $52,53$ & 69 & $52,75$\\ \hline
		70 & $52,29$ & 71 & $52,66$ & 72 & $52,72$ & 73 & $3,75$ & 74 & $3,4$ & 75 & $3,62$ & 76 & $3,70$ & 77 & $61,66$ & 78 & $61,38$ & 79 & $61,62$\\ \hline
		80 & $61,68$ & 81 & $69,72$ & 82 & $69,46$ & 83 & $69,70$ & 84 & $69,68$ & 85 & $139,131$ & 86 & $139,66$ & 87 & $139,136$ & 88 & $139,112$ & 89 & $139,140$\\ \hline
		90 & $135,136$ & 91 & $135,87$ & 92 & $135,62$ & 93 & $135,138$ & 94 & $141,140$ & 95 & $141,116$ & 96 & $141,68$ & 97 & $141,138$ & 98 & $145,133$ & 99 & $145,72$\\ \hline
		100 & $145,144$ & 101 & $145,120$ & 102 & $145,140$ & 103 & $143,144$ & 104 & $143,95$ & 105 & $143,70$ & 106 & $143,138$ & 107 & $53,54$ & 108 & $53,30$ & 109 & $53,58$\\ \hline
		110 & $53,60$ & 111 & $127,79$ & 112 & $127,54$ & 113 & $127,128$ & 114 & $127,130$ & 115 & $103,79$ & 116 & $103,104$ & 117 & $103,108$ & 118 & $103,30$ & 119 & $103,110$\\ \hline
		120 & $131,58$ & 121 & $131,128$ & 122 & $131,104$ & 123 & $131,132$ & 124 & $133,60$ & 125 & $133,130$ & 126 & $133,108$ & 127 & $133,132$ & 128 & $99,100$ & 129 & $99,94$\\ \hline
		130 & $99,98$ & 131 & $99,26$ & 132 & $124,110$ & 133 & $124,100$ & 134 & $124,115$ & 135 & $124,121$ & 136 & $124,51$ & 137 & $118,94$ & 138 & $118,115$ & 139 & $118,117$\\ \hline
		140 & $118,45$ & 141 & $122,98$ & 142 & $122,121$ & 143 & $122,117$ & 144 & $122,49$ & 145 & $50,26$ & 146 & $50,51$ & 147 & $50,45$ & 148 & $50,49$ & 149 & $112,104$\\ \hline
		150 & $112,115$ & 151 & $112,113$ & 152 & $112,39$ & 153 & $112,88$ & 154 & $116,117$ & 155 & $116,113$ & 156 & $116,43$ & 157 & $116,92$ & 158 & $38,45$ & 159 & $38,39$\\ \hline
		160 & $38,43$ & 161 & $38,14$ & 162 & $87,94$ & 163 & $87,88$ & 164 & $87,14$ & 165 & $87,92$ & 166 & $120,108$ & 167 & $120,121$ & 168 & $120,113$ & 169 & $120,47$\\ \hline
		170 & $120,96$ & 171 & $46,49$ & 172 & $46,47$ & 173 & $46,43$ & 174 & $46,22$ & 175 & $95,98$ & 176 & $95,96$ & 177 & $95,92$ & 178 & $95,22$ & 179 & $29,30$\\ \hline
		180 & $29,51$ & 181 & $29,39$ & 182 & $29,47$ & 183 & $29,5$ & 184 & $4,26$ & 185 & $4,5$ & 186 & $4,22$ & 187 & $4,14$ & 188 & $78,79$ & 189 & $78,100$\\ \hline
		190 & $78,96$ & 191 & $78,5$ & 192 & $78,88$ & 193 & $75,54$ & 194 & $75,5$ & 195 & $75,63$ & 196 & $75,71$ & 197 & $66,58$ & 198 & $66,63$ & 199 & $66,39$\\ \hline
		200 & $66,67$ & 201 & $72,60$ & 202 & $72,71$ & 203 & $72,47$ & 204 & $72,67$ & 205 & $62,63$ & 206 & $62,14$ & 207 & $62,65$ & 208 & $70,71$ & 209 & $70,22$\\ \hline
		210 & $70,65$ & 211 & $68,67$ & 212 & $68,43$ & 213 & $68,65$ & 214 & $136,128$ & 215 & $136,63$ & 216 & $136,88$ & 217 & $136,137$ & 218 & $140,132$ & 219 & $140,137$\\ \hline
		220 & $140,113$ & 221 & $140,67$ & 222 & $138,137$ & 223 & $138,92$ & 224 & $138,65$ & 225 & $144,130$ & 226 & $144,71$ & 227 & $144,96$ & 228 & $144,137$ & 229 & $54,6$\\ \hline
		230 & $54,55$ & 231 & $54,57$ & 232 & $30,6$ & 233 & $30,31$ & 234 & $30,35$ & 235 & $30,37$ & 236 & $58,55$ & 237 & $58,31$ & 238 & $58,59$ & 239 & $60,57$\\ \hline
		240 & $60,35$ & 241 & $60,59$ & 242 & $79,80$ & 243 & $79,84$ & 244 & $79,6$ & 245 & $79,86$ & 246 & $128,55$ & 247 & $128,80$ & 248 & $128,129$ & 249 & $130,57$\\ \hline
		250 & $130,84$ & 251 & $130,129$ & 252 & $104,80$ & 253 & $104,105$ & 254 & $104,31$ & 255 & $104,107$ & 256 & $108,35$ & 257 & $108,84$ & 258 & $108,105$ & 259 & $108,109$\\ \hline
		260 & $110,86$ & 261 & $110,107$ & 262 & $110,109$ & 263 & $110,37$ & 264 & $132,59$ & 265 & $132,129$ & 266 & $132,105$ & 267 & $100,86$ & 268 & $100,91$ & 269 & $100,97$\\ \hline
		270 & $100,27$ & 271 & $94,91$ & 272 & $94,93$ & 273 & $94,21$ & 274 & $98,97$ & 275 & $98,93$ & 276 & $98,25$ & 277 & $26,27$ & 278 & $26,21$ & 279 & $26,25$\\ \hline
		280 & $115,107$ & 281 & $115,114$ & 282 & $115,42$ & 283 & $115,91$ & 284 & $121,109$ & 285 & $121,114$ & 286 & $121,48$ & 287 & $121,97$ & 288 & $51,37$ & 289 & $51,27$\\ \hline
		290 & $51,42$ & 291 & $51,48$ & 292 & $117,93$ & 293 & $117,114$ & 294 & $117,44$ & 295 & $45,21$ & 296 & $45,42$ & 297 & $45,44$ & 298 & $49,25$ & 299 & $49,48$\\ \hline
		300 & $49,44$ & 301 & $113,105$ & 302 & $113,114$ & 303 & $113,40$ & 304 & $113,89$ & 305 & $39,31$ & 306 & $39,42$ & 307 & $39,40$ & 308 & $39,15$ & 309 & $88,80$\\ \hline
		310 & $88,91$ & 311 & $88,15$ & 312 & $88,89$ & 313 & $43,44$ & 314 & $43,40$ & 315 & $43,19$ & 316 & $92,93$ & 317 & $92,89$ & 318 & $92,19$ & 319 & $14,21$\\ \hline
		320 & $14,15$ & 321 & $14,19$ & 322 & $47,35$ & 323 & $47,48$ & 324 & $47,40$ & 325 & $47,23$ & 326 & $96,84$ & 327 & $96,97$ & 328 & $96,23$ & 329 & $96,89$\\ \hline
		330 & $22,25$ & 331 & $22,23$ & 332 & $22,19$ & 333 & $5,6$ & 334 & $5,27$ & 335 & $5,23$ & 336 & $5,15$ & 337 & $63,55$ & 338 & $63,15$ & 339 & $63,64$\\ \hline
		340 & $71,57$ & 341 & $71,23$ & 342 & $71,64$ & 343 & $67,59$ & 344 & $67,40$ & 345 & $67,64$ & 346 & $65,64$ & 347 & $65,19$ & 348 & $137,129$ & 349 & $137,89$\\ \hline
		350 & $137,64$ & 351 & $6,7$ & 352 & $6,11$ & 353 & $6,13$ & 354 & $55,7$ & 355 & $55,56$ & 356 & $57,11$ & 357 & $57,56$ & 358 & $31,7$ & 359 & $31,32$\\ \hline
		360 & $31,34$ & 361 & $35,11$ & 362 & $35,32$ & 363 & $35,36$ & 364 & $37,13$ & 365 & $37,34$ & 366 & $37,36$ & 367 & $59,56$ & 368 & $59,32$ & 369 & $80,81$\\ \hline
		370 & $80,7$ & 371 & $80,83$ & 372 & $84,11$ & 373 & $84,81$ & 374 & $84,85$ & 375 & $86,83$ & 376 & $86,85$ & 377 & $86,13$ & 378 & $129,56$ & 379 & $129,81$\\ \hline
		380 & $105,32$ & 381 & $105,81$ & 382 & $105,106$ & 383 & $107,83$ & 384 & $107,106$ & 385 & $107,34$ & 386 & $109,85$ & 387 & $109,106$ & 388 & $109,36$ & 389 & $91,83$\\ \hline
		390 & $91,18$ & 391 & $91,90$ & 392 & $97,85$ & 393 & $97,24$ & 394 & $97,90$ & 395 & $27,13$ & 396 & $27,18$ & 397 & $27,24$ & 398 & $93,90$ & 399 & $93,20$\\ \hline
		400 & $21,18$ & 401 & $21,20$ & 402 & $25,24$ & 403 & $25,20$ & 404 & $114,106$ & 405 & $114,41$ & 406 & $114,90$ & 407 & $42,34$ & 408 & $42,41$ & 409 & $42,18$\\ \hline
		410 & $48,36$ & 411 & $48,41$ & 412 & $48,24$ & 413 & $44,20$ & 414 & $44,41$ & 415 & $40,32$ & 416 & $40,41$ & 417 & $40,16$ & 418 & $89,81$ & 419 & $89,90$\\ \hline
		420 & $89,16$ & 421 & $15,7$ & 422 & $15,18$ & 423 & $15,16$ & 424 & $19,20$ & 425 & $19,16$ & 426 & $23,11$ & 427 & $23,24$ & 428 & $23,16$ & 429 & $64,56$\\ \hline
		430 & $64,16$ & 431 & $7,8$ & 432 & $7,10$ & 433 & $11,8$ & 434 & $11,12$ & 435 & $13,10$ & 436 & $13,12$ & 437 & $56,8$ & 438 & $32,8$ & 439 & $32,33$\\ \hline
		440 & $34,10$ & 441 & $34,33$ & 442 & $36,12$ & 443 & $36,33$ & 444 & $81,8$ & 445 & $81,82$ & 446 & $83,82$ & 447 & $83,10$ & 448 & $85,82$ & 449 & $85,12$\\ \hline
		450 & $106,82$ & 451 & $106,33$ & 452 & $18,10$ & 453 & $18,17$ & 454 & $90,82$ & 455 & $90,17$ & 456 & $24,12$ & 457 & $24,17$ & 458 & $20,17$ & 459 & $41,33$\\ \hline
		460 & $41,17$ & 461 & $16,8$ & 462 & $16,17$ & 463 & $8,9$ & 464 & $10,9$ & 465 & $12,9$ & 466 & $33,9$ & 467 & $82,9$ & 468 & $17,9$ &   &  \\ \hline
	\end{tabular}
\end{table*}


==> Sources/evltn.tex <==
\section{Evaluation}
\label{sec:evaluation}

This is the evaluation part




==> Sources/mdptable.tex <==
\begin{table*}[tp]
	\caption{Mappings between MDP State IDs (Figure \ref{fig:agt}) and Compromised Asset IDs}
	\label{tab:ip-host}
	\centering
	\tiny
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} \\ \hline
		0 & 6 & 1 & 61 & 2 & 610 & 3 & 6102 & 4 & 61023 & 5 & 610234 & 6 & 6102349 & 7 & 61023495 & 8 & 610234957\\ \hline
		9 & 6102349578 & 10 & 610234958 & 11 & 61023497 & 12 & 610234978 & 13 & 61023498 & 14 & 610235 & 15 & 6102354 & 16 & 61023547 & 17 & 610235478\\ \hline
		18 & 61023548 & 19 & 6102357 & 20 & 61023578 & 21 & 6102358 & 22 & 610237 & 23 & 6102374 & 24 & 61023748 & 25 & 6102378 & 26 & 610238\\ \hline
		27 & 6102384 & 28 & 6103 & 29 & 61034 & 30 & 610349 & 31 & 6103495 & 32 & 61034957 & 33 & 610349578 & 34 & 61034958 & 35 & 6103497\\ \hline
		36 & 61034978 & 37 & 6103498 & 38 & 61035 & 39 & 610354 & 40 & 6103547 & 41 & 61035478 & 42 & 6103548 & 43 & 610357 & 44 & 6103578\\ \hline
		45 & 610358 & 46 & 61037 & 47 & 610374 & 48 & 6103748 & 49 & 610378 & 50 & 61038 & 51 & 610384 & 52 & 6104 & 53 & 61049\\ \hline
		54 & 610492 & 55 & 6104925 & 56 & 61049257 & 57 & 6104927 & 58 & 610495 & 59 & 6104957 & 60 & 610497 & 61 & 6105 & 62 & 61052\\ \hline
		63 & 610524 & 64 & 6105247 & 65 & 610527 & 66 & 61054 & 67 & 610547 & 68 & 61057 & 69 & 6107 & 70 & 61072 & 71 & 610724\\ \hline
		72 & 61074 & 73 & 617 & 74 & 60 & 75 & 61024 & 76 & 602 & 77 & 6023 & 78 & 60234 & 79 & 602349 & 80 & 6023495\\ \hline
		81 & 60234957 & 82 & 602349578 & 83 & 60234958 & 84 & 6023497 & 85 & 60234978 & 86 & 6023498 & 87 & 60235 & 88 & 602354 & 89 & 6023547\\ \hline
		90 & 60235478 & 91 & 6023548 & 92 & 602357 & 93 & 6023578 & 94 & 602358 & 95 & 60237 & 96 & 602374 & 97 & 6023748 & 98 & 602378\\ \hline
		99 & 60238 & 100 & 602384 & 101 & 603 & 102 & 6034 & 103 & 60349 & 104 & 603495 & 105 & 6034957 & 106 & 60349578 & 107 & 6034958\\ \hline
		108 & 603497 & 109 & 6034978 & 110 & 603498 & 111 & 6035 & 112 & 60354 & 113 & 603547 & 114 & 6035478 & 115 & 603548 & 116 & 60357\\ \hline
		117 & 603578 & 118 & 60358 & 119 & 6037 & 120 & 60374 & 121 & 603748 & 122 & 60378 & 123 & 6038 & 124 & 60384 & 125 & 604\\ \hline
		126 & 6049 & 127 & 60492 & 128 & 604925 & 129 & 6049257 & 130 & 604927 & 131 & 60495 & 132 & 604957 & 133 & 60497 & 134 & 605\\ \hline
		135 & 6052 & 136 & 60524 & 137 & 605247 & 138 & 60527 & 139 & 6054 & 140 & 60547 & 141 & 6057 & 142 & 607 & 143 & 6072\\ \hline
		144 & 60724 & 145 & 6074 & 146 & 67 &   &   &   &   &   &   &   &   &   &   &   &  \\ \hline
	\end{tabular}
\end{table*}


==> Sources/sec-apndx.tex <==
\section{Appendix}\label{sec:apndx}

\begin{lemma}
\label{LeftCosetsDisjoint}
Let $N$, $C(k)$, and $S(k)$ be the total number of network nodes, compromised set of nodes, and secure (non-compromised) network nodes, respectively. Also, we define $V$ and $\beta(k)$ to be, respectively, the vulnerability factor, and the number of network nodes which get compromised at the $k$-th step during the MDP generation phase. 
Then
\begin{equation}
\beta(k+1) = N\cdot\big(\frac{N-V}{N}\big)^{\frac{\log(1-\frac{C(k)}{N})}{\log(\frac{N-V}{N})}}\cdot\Big[ 1 - \big(\frac{N-V}{N}\big)^{\beta(k)} \Big],
\end{equation}

\end{lemma}

\begin{IEEEproof}
Clearly, the number of internal compromised network nodes is initially zero, i.e., $C(0) = 0$. Given the vulnerability factor of $V$, the next step of the MDP generation will result in $C(1) = V$, i.e., $V$ new MDP states. Next, \name will use each of the $V$ compromised nodes, and the non-compromised hosts which are accessible from any of those $V$ compromised nodes, to further expand the MDP model. It is important to mention that exploration of every compromised node will result in $\leq V$ new compromised nodes as some them may have already been compromised during one of the previous steps. 

We calculate the expected number of non-compromised network nodes which are visited (get compromised) at the $k$-th step of the MDP generation procedure, i.e., $\beta(k+1)$. Clearly, those network nodes are visited through investigation of the nodes which got newly compromised during the previous phase $\beta(k)$. Once the first node out of the $\beta(k)$ nodes is investigated, the expected number of compromised nodes is $E[c_k(1)] = C(k) + V\cdot\frac{N-C(k)}{N}$, where $V\cdot\frac{N-V}{N}$ new nodes are compromised, because $V$ (vulnerability factor) nodes are selected which are each non-compromised with probability $\frac{N-V}{N}$. Following some algebraic calculations and arrangements, we have the closed form solution 
\begin{equation}
c_0(n) = N\cdot\Big[1-\big(\frac{N-V}{N}\big)^{n}\Big],
\end{equation}
and hence, we calculate $\beta(k+1)$ as $C(k+1) - C(k)$:
\begin{equation}
\beta(k+1) = N\cdot\big(\frac{N-V}{N}\big)^\alpha\cdot\Big[ 1 - \big(\frac{N-V}{N}\big)^{\beta(k)} \Big],
\end{equation}
where
\begin{equation}
\alpha = \frac{\log(1-\frac{C(k)}{N})}{\log(\frac{N-V}{N})}.
\end{equation}

\qed
\end{IEEEproof}

==> Sources/sec-index.tex <==

\section{Cyber-physical Security Index}\label{sec:index}

\name uses a new power grid security index to evaluate the security level of each MDP state. The proposed index takes into consideration the severity of the potential malicious physical consequences (i.e. percentage of line overload) and the difficulty to penetrate into the power network. In particular, using a defense-centric metric, \name measures how susceptible the power system is to cyber attack induced contingencies, e.g., line outages, at every MDP state. As explained in the previous section, states capture the set of contingencies that can occur due to malicious actions. Then, \name makes use of an adversary-driven metric to quantify how the attackers can obtain the required privileges to cause those physical contingencies.  Note that the physical contingencies considered here are steady-state contingencies.  Although not discussed, \name could potentially be modified to study transient contingencies as well.

Here, to measure the power system's susceptibility to cyber attack induced contingencies (e.g., line outages) for each state, \name updates the admittance matrix according to the line outages encoded in that state, and solves the AC power flow equations using the iterative Newton-Raphson algorithm to calculate the line flows. Alternatively, an approximate DC model may be used, requiring only a linear solution, but potentially sacrificing detail \cite{dcpowerflowrevisited}.  
% Saman: In traditional power system contingency Analysis, the impacts of contingencies on an electric power system are quantified and finally prioritized.
\name estimates the susceptibility degree using a modified version of the performance index \cite{davis:multipleoutage} that assigns $0$ to a state if there are no line flow violations and a positive value otherwise, computed using the following equation:
\begin{equation}
F(s) =  \sum_{l \in L}  \big[ \max\{\frac{f_s(l)}{f^{MAX}(l)}-1,0 \} \big] ^2.
\end{equation}
Here, $L$ is the set of all lines, $f_s(l)$ denotes flow on line $l$ in state $s$, and $f^{MAX}(l)$ denotes the maximum flow allowed on line $l$.  In the event that a power flow fails to converge, a severe physical impact can be assumed which justifies setting $F(s)$ to a large number, the outage severity.  The outage severity should be much larger than any of the line severity measures.

To calculate the overall cyber-physical security index for each state $I: s \rightarrow \mathbb{R}$, \name uses the above power system performance index in the following dynamic programming equation:
\begin{equation}\label{eq:dynprog}
% I(s) = \max_{a \in A(s)} \{ F(s) + \gamma\cdot\sum_{s' \in S} [P(s'|s,a).I(s')] \},
I(s) = \max_{a \in A(s)} \{\gamma\cdot\sum_{s' \in S} P(s'|s,a)[\Delta F(s,s') + I(s')] \},
\end{equation}
where $I(.)$ (as the MDP's value function) is formulated as a function of difficulty levels of various cyber attack paths $P(s'|s,a)$ and their physical impact $\Delta F(s,s') = F(s') - F(s)$. To solve Equation \eqref{eq:dynprog}, \name implements the value iteration algorithm.  As formulated, proximity of the attacker to a physical component, existence of easy-to-traverse attack paths, and high final physical impacts of the attacks improve the fitness of a system state from the point of view of the adversary.


==> Sources/sec-ovrvw.tex <==
\section{Overview}\label{sec-ovrvw}

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.95\textwidth]{./Figures/Architecture-crop}
  \caption{High-level Architecture of the \name Framework}
  \label{fig:arch}
\end{figure*}


==> The Art of CPU-Pinning-OLD/Sources/PerfStudyanalysis.tex <==

\section{Overhead Analysis of Different Application Types on a Variety of Virtualized Platforms}
\label{sec:PerfStudyanalysis}
\subsection{Evaluation Environment}
In this section, we evaluate the performance of four cloud-based application types (detailed in Table \ref{table:apptypes}) on four popular execution platforms.

\begin{table}[h]
\centering
    \vspace{-2px}
\begin{tabular}{ c|c|c } 
 \hline
 \textbf{Type} &  \textbf{Version} & \textbf{Characteristic} \\
 \hline
 \hline
 FFmpeg & 3.4.6 & CPU-bound workload\\
 Open MPI & 2.1.1 & HPC workload \\ 
 WordPress & 5.3.2 & IO-bound web-based workload \\ 
 Cassandra & 2.2 & Big Data (NoSQL) workload \\ 
  \hline
\end{tabular}
\caption{\small{Specifications of application types used for evaluation.} }
\label{table:apptypes}
   \vspace{-5px}
\end{table}

The performance metric we measure in the evaluations is the \emph{execution time} of each application type. Also, to quantify the overhead of a certain virtualized platform, we define \emph{overhead ratio} as the average execution time offered by a given virtualized platform to the average execution time of bare-metal. 
Table \ref{table:hwconfig} describes the configuration of instance types used for the evaluation. The host server is a DELL PowerEdge R830 with 4$\times$Intel Xeon E5-4628Lv4 processors with 112 homogeneous cores, 384 GB memory (24$\times$16 GB DRAM), and RAID1 (2$\times$900 GB HDD) storage. Each processor is 1.80 GHz with 35 MB cache and 14 processing cores (28 threads).

\begin{table}[h]

\centering
\begin{tabular}{ c|c|c } 
 \hline
\textbf{Instance Type} &  \textbf{No. of Cores} & \textbf{Memory (GB)} \\
 \hline\hline
 \texttt{Large} & 2 & 8 \\
 \texttt{$\times$Large} & 4 & 16 \\ 
 \texttt{2$\times$Large} & 8 & 32 \\ 
 \texttt{4$\times$Large} & 16 & 64 \\ 
 \texttt{8$\times$Large} & 32 & 128\\
 \texttt{16$\times$Large} & 64 & 256\\
  \hline
\end{tabular}
\caption{\small{List of instance types used for evaluation.}}
\label{table:hwconfig}
   \vspace{-5px}
\end{table}


The four studied execution platforms include bare-metal, which imposes the minimum overhead and is used as the baseline, in addition to three variations of virtualized platforms commonly used in the cloud (\ie VMs, containers, and containers within VMs). Figure \ref{Fig:Platforms} provides a schematic view of the four execution platforms and Table~\ref{table:config} elaborate on the specifications of each platform. The abbreviations mentioned in the table are used henceforth to represent each execution platforms. Note that each execution platform can be instantiated using any instance type of Tabel~\ref{table:hwconfig}. 

\begin{table}[hb]
\vspace{-2px}
\centering
\begin{tabular}{ c|c|l } 
 \textbf{Abbr.} & \textbf{Platform} &  \textbf{Specifications} \\
 \hline
 \hline
 BM & Bare-Metal & \small{Ubuntu 18.04.3, Kernel 5.4.5} \\
 \hline
VM & \small{Virtual Machine} & \small{Qemu 2.11.1, Libvirt 4}\\
& &\small{Ubuntu 18.04.3, Kernel 5.4.5} \\
\hline
 CN & \small{Container on} & \small{Docker 19.03.6}, \\
 & \small{Bare-Metal} & \small{Ubuntu 18.04 image} \\ 
 \hline
VMCN & \small{Container on VM} & \small{As above}\\
\end{tabular}
\caption{\small{Characteristics of different execution platforms used in the evaluations. First column shows the abbreviation of the execution platform used henceforth in the paper.}}
\label{table:config}
\end{table}


\begin{figure*}[t]
  \centering
  \includegraphics[width=0.8\textwidth]{Figures/Platforms.pdf}
  \caption{The four execution platforms used for performance evaluation of different application types.}
  \label{Fig:Platforms}
  \vspace{-0.2in}
\end{figure*}

% Docker will be used as container technology and Linux KVM will be used as the hypervisor for VMs. 


Bare-metal (BM) execution platform only includes the host OS and the application. In VM platform, one Ubuntu VM instance is created (based on KVM hypervisor) to process requests of the application type in question. 
Similarly, in container platform (CN), one Docker container is instantiated on bare-metal from an Ubuntu image. Lastly, VMCN platform refers to an execution platform where a Docker container is instantiated within a VM (with the aforementioned configurations).

Resource contention between coexisting processes in a host can potentially affect the tasks' execution times, hence, introducing noise in our overhead measurement objective. To avoid such noises, we assure that 
each application type is examined in isolation. That is, during the evaluation process, there is no other coexisting workload in the system.

As for the performance monitoring tools employed in this study, we used basic Linux utilities, such as \texttt{top, htop, iostat} and \texttt{perf}, alongside with \texttt{BCC} (BPF Compiler Collection \cite{BCC}) as a profiling tool to perform kernel tracing and to track the execution status of processes running inside the OS. In particular, we used \texttt{cpudist} and \texttt{offcputime} to monitor and profile the instantaneous status of the processes in the OS scheduler.

%It is proven that scheduling is a source of overhead in any execution platform \cite{}.
Irrespective of the execution platform, the host OS scheduler is the ultimate decision maker in allocating processes to CPU cores \cite{wong2008fairness}. A process (\eg \texttt{FFmpeg}) can be potentially assigned to a different set of cores at each scheduling event. It is important to note that even VMs are considered as processes from the host OS perspective. 

As the scheduling events happen frequently and there are numerous cores in a typical cloud host, migrating processes from one core to another at each event is expected to induce a remarkable overhead in the cloud hosts. Specifically, among other reasons, migrating a given process induces overheads for redundant memory access due to cache miss, reestablishing interrupts for IO operation, and context switching \cite{wong2008fairness,qiu2017lxc}. Even more overheads are involved in migrating virtualized platforms, \eg for resource usage accounting activities.

We need to measure and verify the significance of the induced overhead of different execution platforms on the overall performance. We envisage that overriding the host OS scheduler, via \emph{CPU pinning} techniques, limits process migrations to a smaller set of CPU cores, hence, reduces the imposed overhead. As such, to verify the impact of CPU pinning, we evaluate each execution platform for different workloads with and without CPU pinning. Note that the virtualized platforms offer built-in pinning ability (\eg via $Qemu$ configuration file for each VM). For BM, we modelled pinning via limiting the number of available CPU cores on the host using GRUB configuration in Linux \cite{marshall2001boot}.

%SHOULD WE EMPHASIZE THAT WE CONSIDER ONLY CPU AND NOT IO OR MEMORY OVERHEAD???

\subsection{Application-Specific Overhead Analysis}

In the following subsections, we concentrate on the characteristics of each application type across different execution platforms. Later, in Section~\ref{sec:cross}, we provide a collective cross-application overhead analysis on the root causes of the imposed overhead. 

\subsubsection{Video Processing Workload Using FFmpeg}\label{subsec:ffmpeg}
FFmpeg offers a wide variety of video transcoding functions, such as those to change video resolution, bit-rate, frame rate, and compression standard. Changing the compression standard (a.k.a \emph{codec}) is known to be the most CPU-intensive transcoding operation \cite{CVSSJournal,analysistpds18} with small memory footpring (around 50 MB in our observations). Hence, we employ it in this study to represent a CPU-intensive workload. This also makes the overhead of the execution platform more visible and makes it easier to harvest. FFmpeg is a multi-threaded application and can utilize up to 16  CPU cores to transcode a video. Hence, for this evaluation, we do not allocate more than 16 cores (\ie \texttt{4$\times$large}) to each execution platform. 

We examine a source video segment\footnote{The video file is free-licensed and is publicly available in the following address:~\url{https://peach.blender.org/download/}} that has a large codec transcoding time. The reason that we examine one video segment is to concentrate on the overhead resulted from the execution platform and remove any uncertainty in the analysis, caused by the video characteristics. 
The source video segment is 30 MB in High Definition (HD) format. The codec is changed from AVC (\texttt{H.264}) to HEVC (\texttt{H.265}). The evaluation was conducted 20 times and the mean and confidence interval of the results were collected. 
%%%%%%% MP4 is media container, H264 is AVC
%The source video segment is 30 MB in High Definition (HD) format. The codec is changed from MP4 (\texttt{H.264}) to HEVC (\texttt{H.265}). The evaluation was conducted 20 times and the mean and confidence interval of the results were collected. 




Results of the evaluation is shown in Figure~\ref{Fig:FFmpeg-all} where the vertical axis shows the mean execution time for each experiment and the horizontal axis shows different instance types. We note that the confidence interval in many cases were negligible. 

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/FFmpeg-all.pdf}
  \caption{\small{Comparing execution time of FFmpeg on different execution platforms under varying number of CPU cores. Horizontal axis indicates the number of CPU cores in form of different instance types.}}
  \label{Fig:FFmpeg-all}
   \vspace{-0.1in}
\end{figure}

% FFmpeg is an absolute CPU-bound application making the expectation to clearly identify CPU performance penalties made by virtualization layers. 
Specific observations and analysis of Figure~\ref{Fig:FFmpeg-all} are enumerated in the following list. Note that, we defer further analysis of these observations to Section~\ref{sec:cross} where we conduct a comparative study across all application types. 

\begin{enumerate}[label=\roman*.]
\item VMCN imposes the highest overhead and pinning it cannot reduce the overhead remarkably. Alternatively, CN platforms (particularly, pinned CN) are shown to impose the minimal overhead with respect to BM. Importantly, we observe that as the number of cores increases, the overhead of vanilla CN and both VMCN platforms decrease. 

\item The imposed overhead of VM platforms (vanilla or pinned) across all instance types is remarkable to the extent that causing the execution times to remains at least twice as much as BM. Unexpectedly, pinning does not mitigate the imposed overhead for VMs when FFmpeg application is deployed.

\item By adding the containerization layer on top of VM (\ie VMCN), even a larger performance overhead is imposed. The maximum and minimum imposed overhead ratios are 4 and 1, respectively. However, as the number of CPU cores allocated to the VMCN increases, the overhead is mitigated drastically, such that for \texttt{4$\times$Large}, the overhead imposed by VMCN is almost the same as VM. Furthermore, overhead ratio of VM and VMCN (vanilla and pinned) remains almost the same across all instance types.

\item Unlike VM and VMCN, pinning CN significantly reduces the overhead, particularly when containers are allocated with fewer processing cores (\eg \texttt{Large}). This suggests that pinned CN is a suitable virtualization platform for CPU-bound applications, such as FFmpeg. 

\end{enumerate}
   
\subsubsection{Parallel Processing Workload Using MPI} 
Message Passing interface (MPI) \cite{gropp1999using} is a widely-used high performance computing (HPC) platform to develop parallel programs. For the analysis, we examined two MPI applications, namely \emph{MPI\_Search} (for parallel searching of an integer value) \cite{FSU} and \emph{Prime\_MPI} \cite{FSU2} (to find all prime numbers within a given range). In these applications, the communication part dominates the computation part. This is to enable us concentrating on the impact of various virtualization platforms on the overall overhead imposed, in circumstances where intensive communication occurs between cores of the same virtualized platform. As our observations for both of the MPI applications were alike, to avoid redundancy, we only report the results for MPI\_Search. To remove any randomness in the results, the evaluations were conducted 20 times and the mean and confidence interval of the execution times are reported. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/MPI-all.pdf}
  \caption{\small{Comparing execution time of MPI\textunderscore search on different execution platforms. Horizontal axis represents the number of CPU cores in the form of different instance types. Vertical axis shows the mean execution time (in seconds).}}
  \label{Fig:MPI-all}
   \vspace{-5px}
\end{figure}



Result of this evaluation is shown in Figure \ref{Fig:MPI-all}. %Vertical axis shows the mean execution time (in seconds) and horizontal axis shows different instance types. 
%%%%%%We already explaining the axis on the figure caption already
Our observations and analyses are as follows:
\begin{enumerate}[label=\roman*.]
\item Overhead imposed by VMCN platforms (both vanilla and pinned) is slightly more than VM-based platforms. Surprisingly, the overhead of CN (vanilla and pinned) even exceeds the VMCN platforms. A closer observation reveals that, for the MPI applications, the overhead of any containerized platform exceeds the ones for the VM platforms.
Although the difference in the imposed overheads is reduced for larger number of cores, the overhead ratio remains the same.

\item From \texttt{2$\times$Large} onward, we notice that the overhead of VM platforms (vanilla and pinned) becomes negligible and the execution times become almost the same as BM. The reason is that, as we move towards larger instances, the bottleneck shifts from computation part to the communication part. Because the hypervisor (KVM) provides an abstraction layer to facilitate inter-core communication between VM's cores, the imposed overhead diminishes and their execution times approach BM. This is unlike communications within cores of a container that involves host OS intervention, thus, implies a higher overhead \cite{ZhengLi}. It is noteworthy that for smaller instance types, the bottleneck of VM platforms is in the computation part that, due to several abstraction layers, incurs a significant overhead.

\end{enumerate}

\subsubsection{Web-based Workload Using WordPress}
WordPress is a PHP-based content management system (CMS) that uses Apache Web Server and MySQL database in the back-end. It is broadly deployed in clouds %\cite{patel2011performance} 
and known to be IO intensive \cite{patel2011performance}, because each HTTP request to a website implies at least network (to read/write from/to the socket) and disk IO (to perform file/database operations). As such, we consider it as a representation of an IO intensive application, in which each process receives at least three IO interrupts. 

We configured the same WordPress website on all of the execution platforms. Apache Jmeter \cite{Jmeter} is a tool to apply workload and measure the performance of a web server. We configured it to generate 1,000 simultaneous web requests (\ie processes) on each execution platform and then, we calculated the mean execution time (a.k.a \emph{response time}) of these web processes. We note that Jmeter itself is a resource intensive application that can affect our intended performance evaluation. Therefore, we configured it to run on a dedicated server in the same network. To remove any possible environmental randomness, we evaluated the workload six times on each instance type. Then, we report the mean and 95\% confidence interval of response time of all web requests.

\begin{figure}[b]
 \vspace{-7px}
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/Wordpress-all.pdf}
  \caption{\small{Comparing mean response time (aka execution time) of 1,000 web processes on different execution platforms (WordPress evaluation). The horizontal axis represents the number of CPU cores in the form of different instance types and the vertical axis shows the mean execution time (in seconds).}}
  \label{Fig:Wordpress-all}

\end{figure}

Results of this evaluation are shown in Figure \ref{Fig:Wordpress-all}. The vertical axis shows the mean execution time of 1,000 web processes (in Seconds) and the horizontal axis shows different instance types. Our observations and analyses of the results are enumerated in the following list: 

\begin{enumerate}[label=\roman*.]
\item Unlike pinned CN that imposes the lowest overhead, vanilla CN imposes the highest overhead across all execution platforms---twice as much as BM for \texttt{Large} instance type. However, by increasing the number of CPU cores, this behavior is changed such that the mean execution time offered by vanilla CN approaches BM. As a similar behavior is observed for other application types, we defer analysis of this observation to Section~\ref{sec:cross}.

\item Even though VMCN platforms (vanilla and pinned) include one more layer of virtualization in compare with VM platforms, they impose a slightly lower overhead. Further analysis within VM platforms shows that the pinned VM consistently imposes a lower overhead than the vanilla VM. Building upon these two observation, we hypothesize that, for IO intensive applications, both pinning and containerization are decisive factors in mitigating the imposed overhead of the virtualized platform. In curtail, the reason that pinning remarkably mitigates the execution time overhead is a more efficient use of the cache and the possibility to pin virtualized platforms on CPU slots based on their IO affinity \cite{pinning}. Alternatively, in a non-pinned (\ie vanilla) scenario, at each time slot, the virtualized platform is allocated on a different set of processing cores by the scheduler that may not favor IO affinity and implies reestablishing the cache. We elaborate this analysis further in Section~\ref{sec:cross} with respect to other application types as well.

% This suggests that container technology can help virtualization to handle IO more efficiently, and by leveraging pinning (pinned VMCN), even more improvement is achieved.


\end{enumerate}

\subsubsection{NoSQL Workload using Apache Cassandra}
Apache Cassandra \cite{abramova2013nosql} is a distributed NoSQL database extensively used to handle Big Data in the cloud. We evaluate it in this study as an application type that demands compute, memory, and IO. We configured Cassandra exclusively on one execution platform and used its native stress tool, \emph{Cassandra-stress} \cite{shirinbab2017performance}\cite{abramova2013nosql}, to submit 1,000 synthesized database operations within one second. A set of 100 threads, each one simulating one user, were spawned by Cassandra-stress. To make the imposed overhead stand out, we put Cassandra under extreme pressure by forcing a quarter of the synthesized requests as the \emph{write} operations and the rest as the \emph{read} operations. Then, we calculated the average execution time (a.k.a response time) of all the synthesized operations. To capture the randomness in the results, caused by the execution platforms, we conducted the experiment 20 times for each instance type and the mean and 95\% confidence interval of the results are reported.

\begin{figure}[b]
 \vspace{-7px}
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/Cassandra-all.pdf}
  \caption{\small{Comparing mean execution time (aka response time) of Cassandra workload (in seconds) on different execution platforms. Horizontal axis represents the number of CPU cores in the form of different instance types. Note that the execution time for the \texttt{Large} instance type is out of range and unchartable. }
  \label{Fig:Cassandra-all}}
\end{figure}

Results of this evaluation are shown in Figure \ref{Fig:Cassandra-all}. Note that, for the \texttt{Large} instance type, the system is overloaded and thrashed and the results are out of range. As such, to be able to concentrate on the imposed overhead of other instance types, we excluded the results of the \texttt{Large} type. Our observations and analysis for this experiment are as follows: 

\begin{enumerate}[label=\roman*.]
\item Vanilla CN imposes the largest overhead---3.5 times or more with respect to BM. This overhead is even higher than the similar phenomenon we observed for WordPress (in Figure~\ref{Fig:Wordpress-all}). The reason for this behavior is the higher volume of IO operations in Cassandra rather than WordPress. However, the CN overhead diminishes for instances with larger number of cores. As we had similar observations for other application types, we defer further analysis of this phenomenon to Section~\ref{sec:cross}. 

\item In contrast to vanilla CN, pinned CN imposes the lowest overhead. This confirms our earlier observations on the positive impact of pinning on IO intensive applications. Surprisingly, we see that for \texttt{$\times$Large}---\texttt{4$\times$Large} instance types, pinned CN can even beat BM. The reason is the BM scheduler is oblivious to IO affinity and the extreme volume of IO operations makes BM perform worse than the pinned CN. For the same reason, we can see that offering a lower execution time is not limited to only pinned CN, but it is also noticed in any pinned virtualized platform.

\item By increasing the number of cores, the impact of pinning is diminished to the extent that for \texttt{8$\times$Large} and \texttt{16$\times$Large} instance types, there is no improvement between the pinned virtualized platforms and their vanilla counterparts. We believe this is because in virtualized platforms with larger instance types: (A) there are fewer scheduling options within the host machine, hence, the scheduling overhead is mitigated; (B) cache and IO affinity are improved, because in each scheduling time slot, it is likely that a virtualized platform is assigned to the same set of processing cores.

\item For all VM-based platforms whose instance type is \texttt{8$\times$Large} and beyond, there is an increased overhead with respect to BM. As noted in the previous point, for larger instances, the overhead of IO diminishes, hence, the execution time is dominated by the CPU processing time. This makes the situation similar to CPU intensive application types (\eg FFmpeg) where VM-based platforms impose a considerable overhead. 

% \item VMCN platforms (vanilla or pinned) show better performance comparing to VM platform (vanilla or pinned). This indicates that container technology helps virtualization to handle IO with less overhead, which is observed in Wordpress evaluation as well. THERE IS A BIG WAY HERE..
\end{enumerate}

\section{Cross-Application Overhead Analysis}\label{sec:cross}

Building upon application-specific observations conducted in the previous section, in this part, we further analyze the root causes of the imposed overhead by various virtualization platforms across different application types. We also carry out additional experiments to verify our findings.

By comparing the results and studying overhead behavior across all application types and execution platforms, the following two categories of the imposed overhead can be distinguished:
% \begin{enumerate}
\paragraph*{1) \textbf{Platform-Type Overhead (PTO)}}
This kind of overhead pertains to the type of virtualized platform and its ratio remains constant, irrespective of the instance type it is deployed on. For instance, in both FFmpeg (Figure~\ref{Fig:FFmpeg-all}) and Cassandra (for instance types greater than \texttt{4$\times$Large} in Figure~\ref{Fig:Cassandra-all}), the overhead ratio of VM remains the same across various instance types. This type of overhead is caused by the abstraction layers of the virtualized platforms and are reflected when CPU intensive applications (\eg FFmpeg) are deployed. As the source of this type of overhead pertains to virutalization layers, pinning cannot mitigate it drastically. This type of overhead is a known issue and has been studied in prior works \cite{felter2015updated,ccpe14amini,spe14amini}.

\paragraph*{2) \textbf{Platform-Size Overhead (PSO)}}
This type of overhead is diminished by increasing the number of cores assigned and is specific to vanilla CN platform. PSO is observed throughout all the studied application types, particularly, when a container is assigned a small portion of the host CPU cores. Our hypothesis is that the ratio of the container cores to the host cores is a decisive factor on the magnitude of the imposed overhead. This behavior of containers has also been identified and reported for Docker by IBM~\cite{IBM}. In particular, for IO-bound applications, the overhead even exceeds VM platforms. As an instance, for \texttt{Large} instance type, the overhead ratio of vanilla CN to vanilla VM for WordPress application is 2.4 (see Figure~\ref{Fig:Wordpress-all}) and it is 3.7 for Cassandra (see Figure~\ref{Fig:Cassandra-all}). Importantly, pinning can considerably mitigate this type of overhead. Since this type of overhead has not been investigated before, we elaborate on its root causes in the next subsections. 

\subsection{The Impact of Container-to-Host Core Ratio (CHR) on PSO}
To analyze the impact of container size on PSO, for a given container, we define \emph{Container-to-Host Core Ratio} (CHR) as the ratio of its assigned cores to the total number of host cores. To evaluate the impact of CHR, we choose FFmpeg as the application type, because it does not impose additional IO overhead and our analysis is concentrated on PSO.
We configure a CN platform of \texttt{4$\times$Large} type on two homogeneous hosts, with 16 and 112 cores, respectively. Then, we measure the mean execution time of the FFmpeg workload (described in Section~\ref{sec:PerfStudyanalysis}) on these configurations. 

\begin{figure}[b]

  \centering
  \includegraphics[width=0.45\textwidth]{Figures/16coreBM.pdf}
  \caption{\small{Evaluating the impact of CHR on the overhead of a vanilla and a pinned CN platform on two homogeneous hosts with 16 and 112 cores. The vertical axis shows the mean execution time (in seconds) and the horizontal axis shows the host's number of cores.}}
  \label{Fig:16coreBM}
      \vspace{-7px}
\end{figure}

Results of this experiment are shown in Figure \ref{Fig:16coreBM}. 
%The vertical axis shows the mean execution time of a vanilla and a pinned  \texttt{4$\times$Large} CN platform (in seconds) and the horizontal axis shows hosts with different number of cores. That is,
The first set of bars represent CHR=1 and the second set represent CHR=0.14. In addition to the CN platform, we report the result for the BM platform with 16 cores. This enables us to study the overhead of a CN platform that is as big as the host machine.



In this figure, we observe that although the CN platforms have the same number of cores, on the larger host (with 112 cores) they impose a higher overhead in compare with the case that they are deployed on the smaller host. We can conclude that a container with a lower value of CHR imposes a larger overhead (PSO) to the system. As illustrated in the figure, pinning does not imply any statistically significant difference in the imposed overhead.

Throughout Section~\ref{sec:PerfStudyanalysis}, we repeatedly observed  the impact of increasing CHR on mitigating PSO across different application types. That is, for larger CN platforms, the execution time approaches BM, even more rapidly than other virtualized platforms. 

The question arises in this case is that, for a given container that processes a certain application type, how to know the suitable value of CHR? In this work, we address this question based on our observations for different application types. However, we note that answering this question theoretically is an interesting future research work. 
In WordPress, the PSO starts to vanish when the CN is configured in the range of [\texttt{4$\times$Large} , \texttt{8$\times$Large}] that implies $0.14 < CHR < 0.28$. A similar observation was made in the IBM report for their proprietary IBM WebSphere web server \cite{IBM}. Similar analysis for FFmpeg and Cassandra indicate suitable CHR should be in the range of $0.07 < CHR < 0.14$ and $0.28 < CHR < 0.57$, respectively. From this analysis, we conclude that IO intensive applications require a higher CHR value than the CPU intensive ones.
%The conclusion drawn from this analysis is summarized in the following insight.
%\begin{shaded*}
%\noindent\textbf{Insight.} %IO intensive applications require a higher range of CHR values whereas CPU intensive applications are the opposite. 
%Alternate version below
%IO intensive applications require a higher CHR value than CPU intensive applications
%\end{shaded*}

The estimated ranges of CHR can be used by cloud administrators to configure containers such that their imposed overhead is minimized. This can potentially benefit both cloud users (by reducing their incurred cost and response time) and cloud providers (by lowering their energy consumption).

\subsection{The Impact of Container Resource Usage Tracking on PSO}
Although CHR explains the diminishing PSO for containers with larger instances, it does not explain the high PSO of small vanilla CNs (\ie those with low CHR) that we observed for all task types. Recall (from Figures \ref{Fig:FFmpeg-all}, \ref{Fig:Wordpress-all}, and \ref{Fig:Cassandra-all}) that pinning remarkably mitigate the PSO for low-CHR CNs. Accordingly, our hypothesis is that the high PSO is attributed to CPU provisioning model. 

We observed in our experiments that, for small vanilla CN (those with 2 cores), \os~scheduler allocates all available CPU cores of the host machine (112 cores) to the CN process. In this circumstance, cgroups has to assure that the cumulative CPU usage of the process does not exceed its designated quota. This means that in each scheduling event, vanilla CN undergoes the overhead of both OS scheduling (that implies process migration) and cgroups (for resource usage tracking). We realized that cgroups is an atomic (kernel space) process \cite{Kernel.org-cgroup}\cite{Josef} and each invocation of it implies one transition from the user-mode to the kernel-mode, which incurs a considerable overhead. Furthermore, we noticed that, in amortizing the process of a small container across all available CPU cores, the process footprint on each core is a tiny fraction of the whole process. Specifically, for small containers, we observed that the overhead of cgroups tasks reaches to the point that it dominates the container process. In particular, because cgroups is an atomic process, the container has to be suspended, until tracking and aggregating resource usage of the container is complete. 

In contrast to the vanilla mode, CPU pinning avoids the overhead of host \os~scheduling and cgroups. In the presence of pinning, as the allocated set of processing cores do not change at each scheduling event, there is less demand for cgroups invocation, hence, the imposed overhead is mitigated. 

\subsection{The Impact of IO Operations on PSO}
The comparison of FFmpeg (particularly, \texttt{$\times$Large} in Figure \ref{Fig:FFmpeg-all}) against WordPress and Cassandra (particularly, \texttt{$\times$Large} in Figures \ref{Fig:Wordpress-all} and \ref{Fig:Cassandra-all}) illustrates that, in both WordPress and Cassandra, the PSO of vanilla CN (\ie the overhead part, colored in \textcolor{red}{red}) is drastically higher than FFmpeg. As both WordPress and Cassandra are IO-bound applications, our hypothesis is that the extra overhead pertains to performing the IO operations.

As a CPU-bound application, FFmpeg has a predictable behavior and fully utilizes their CPU quota in each time slot. In contrast, the IO-bound applications often do not make a complete use of their CPU quota, because they are interrupted and switch to the  \emph{pending} state, until they complete their IO operation. For example, in WordPress, each web request triggers at least three Interrupt Requests (IRQs): to read from the network socket; to fetch the requested HTML file from disk; and to write back to the network socket. Each IRQ implies the overheads to accomplish a set of scheduling actions (to enqueue, dequeue, and pick the next task %\cite{}
) and transitioning to the kernel mode (to perform the IO operation).
% In the case of FFmpeg, the OS scheduler calculates weight based on a load average calculation, and it degrades this calculation based on time. FFmpeg is almost never going to take itself off the CPU voluntarily until the task is finished, which makes its scheduling decisions very simple. Its historical load average will be basically the same as its next run load average, because again, it just want to use all the CPU it possibly can. 
%In the case of WordPress application, Apache and MySQL processes are heavily IO demanding. An HTTP . 

Once an interrupt is served, to avoid cache line bouncing and reestablishing IO channels, OS scheduler makes its best effort to resume the interrupted tasks on the same set of cores. However, in the event that the process is assigned to a different set of cores, a significant overhead is imposed to reload L1 and L2 caches and establish new IO channels. As noted in the previous section, vanilla CN instances with smaller CHR are more prone to be allocated on a different set of cores, hence, experiencing even a more significant overhead, when compared with larger instances. 

\subsection{The Impact of Multitasking on PSO}
Analysis of the overhead across different application types, in particular FFmpeg versus WordPress, brings us to the hypothesis that the number of processes increases the imposed PSO. To verify the hypothesis and figure out the importance of this factor, in this part, we conduct an experiment to analyze the impact of number of FFmpeg processes on its PSO. The reason that we compare FFmpeg with itself is to eliminate the impact of differences in application characteristics and, instead, single out the impact of number of processes. 

For this experiment, we examined FFmpeg on \texttt{4$\times$Large} CN instance types to change the codec of the video file used in Section~\ref{subsec:ffmpeg}. We studied two scenarios: (A) the source video file is a 30-second (large) video; and (B) splitting the same source video into 30 video files of the same size (one-second each) and process them in parallel.



Comparing the results in Figure~\ref{Fig:LargeSmall} approves our hypothesis and shows that the number of processes results in increasing the PSO of CN platforms. This is because, a higher degree of multitasking increases the overhead imposed by OS scheduler and cgroups to collect resource usage of CNs.  




 \begin{figure}[h]
   \vspace{-3px}
  \centering
  \includegraphics[width=0.45\textwidth]{Figures/LargeSmallTasks.pdf}
  \caption{\small{Comparing the impact of number of processes on the imposed overhead of \texttt{4$\times$Large} CN instance. The vertical axis shows the mean executing times (in Seconds) and the horizontal axis shows processing of a source video file in two cases: one large video versus partitioning it into 30 small videos.}}
  \label{Fig:LargeSmall}
  \vspace{-5px}
\end{figure}

 











==> The Art of CPU-Pinning-OLD/Sources/abs.tex <==
\begin{abstract}

%Throughout the last decade, virtualization platform technologies have evolved---from Virtual Machines (VMs) to various forms of containers---and have become an indispensable part of the cloud computing industry.
Cloud providers offer a variety of execution platforms in form of bare-metal, VM, and containers. However, due to the pros and cons of each execution platform, choosing the appropriate platform for a specific cloud-based application has become a challenge for solution architects. The possibility to combine these platforms (\eg deploying containers within VMs) offers new capacities that makes the challenge even further complicated. However, there is a little study in the literature on the pros and cons of deploying different application types on various execution platforms. In particular, evaluation of diverse hardware configurations and different CPU provisioning methods, such as CPU pinning, have not been sufficiently studied in the literature. In this work, the performance overhead of container, VM, and bare-metal execution platforms are measured and analyzed for four categories of real-world applications, namely video processing, parallel processing (MPI), web processing, and No-SQL, respectively representing CPU intensive, parallel processing, and two IO intensive processes. 
Our analyses reveal a set of interesting and sometimes counterintuitive findings that can be used as best practices by the solution architects to efficiently deploy cloud-based applications. Here are some notable mentions: (A) Under specific circumstances, containers can impose a higher overhead than VMs; (B) Containers on top of VMs can mitigate the overhead of VMs for certain applications; (C) Containers with a large number of cores impose a lower overhead than those with a few cores. %overhead depends on the ratio of the CPU cores allocated to it to the total number of available cores to host.

%Our evaluations reveal that: (A) the overhead imposed by different virtualized platforms varies depending on the application characteristics; (B) CPU pining can reduce the overhead of virtualized platforms, particularly, for containers; and (C) in a cloud host, the proportion of CPU cores allocated to a container to the total number of available cores is a decisive factor on the virtualization overhead. %****. talk about proportion of pinning considerable effects of CPU pinning is studied.
\end{abstract}

\begin{IEEEkeywords}
Virtualization, Container, performance overhead, CPU pinning.
\end{IEEEkeywords}



==> The Art of CPU-Pinning-OLD/Sources/ack.tex <==
\section*{Acknowledgment}
\small{We thank reviewers of the manuscript. The research was supported
by the Louisiana Board of Regents under grant number LEQSF (2017-
20)-RD-B-06, Perceptive Intelligence LLC, and Amazon Cloud (AWS) research credit.}

==> The Art of CPU-Pinning-OLD/Sources/background.tex <==

\section{Background}
\label{sec:background}
\subsection{Overview}
% In general, any means by which many different users are able simultaneously to interact with a computing system while each perceiving that they have an entire execution environment to themselves, is a form of virtualization\cite{Gautam-virtualization}. 
Virtualization platforms emulate and isolate compute, storage, and network resources within a host. Current virtualization platforms are categorized based on the level of abstraction they provide. In particular, VMs provide a hardware layer abstraction, known as \emph{hardware virtualization}, whereas containers enable abstraction from the operating system (OS) layer, known as \emph{OS virtualization} \cite{BuyyaMasteringBook}.


%%%%%%%%%% Figure moved to Intro

% \paragraph*{Hardware virtualization} 
\subsection{Hardware Virtualization (VM)} 
Hardware virtualization operates based on a hypervisor that enables one or more isolated guest operating systems (VMs) on a physical host \cite{ppACSC,salehi2011contention}. KVM \cite{felter2015updated} is a popular open-source hypervisor extensively used by cloud providers. For instance, AWS developed a KVM-based hypervisor called \emph{Nitro} \cite{awsnitro} and uses it for its \texttt{C5} VM types. Many datacenter management platforms have been developed around KVM hypervisor. For instance, Hyper Converged Infrastructure (HCI) platforms \cite{Hci} (\eg Nutanix \cite{Nutanix}, Maxta \cite{Maxta}, and Cloudistics \cite{Cloudistics}) that enable integrated software defined datacenters have adopted KVM as their underlying hypervisor.

KVM hypervisor, depicted in Figure~\ref{fig:KVMarch}, is part of the host kernel and works directly with hardware virtualization features (\eg \texttt{Intel-VT} and \texttt{AMD-v} \cite{goto2011kernel}) to share the hardware resources across multiple fully isolated VMs. KVM interfaces with the user space (\eg via \texttt{QEMU}) and executes guest OS commands via \texttt{ioctls} kernel module. Qemu-KVM emulates hardware devices for VMs and can para-virtualize \cite{goto2011kernel} IO devices, such as disk and NIC, by using specific drivers that expedite accessing them. \texttt{Libvirt} is a library to help external services to interact with KVM/QEMU using its APIs. \texttt{virsh} and \texttt{virt-manager} are command-line and GUI interfaces for Libvirt. 

\subsection{OS Virtualization (Container)} 
Container is a lightweight and portable virtualization solution in which the host OS kernel is shared across multiple isolated user-space environments. In contrast to VMs, containers are transparent from the host OS perspective. That is, the processes created by a container are visible to the host OS as native processes, however, the container itself is not a process. All processes created via a container have access to the same set of resources and libraries. 

Technically speaking, a container is an abstraction created by the coupling of \emph{namespace} and \emph{cgroups} modules of the host OS. A namespace that is assigned to a container creates an abstraction for the processes of the container and offers them an isolated user space, such as network configurations, storage space, and software packages. 
% namespace shares the kernel with the host that makes it a light weighted OS virtualization solution. 

Control Groups (a.k.a \texttt{cgroups}) is a kernel module that enforces and monitors resource usage limitations for a given group of processes \cite{Kernel.org-cgroup}\cite{Josef}. Cgroups module of the host OS is in charge of enforcing resource constraints designated for a container instance. As an example, for a container instance with two CPU cores, cgroups oversees its usage not to go beyond the two cores across the entire host. It is noteworthy that the way cgroups enforces constraints is a decisive factor from the performance overhead perspective.





Docker \cite{yu2015live} is the most widely adopted container technology in the cloud era, hence, we consider it as the container platform in this study. However, we believe that our findings can be extrapolated to other containerization techniques that operates based on cgroups (\eg Singularity). Figure~\ref{fig:DockerArch} illustrates the architecture of the Docker container. Docker Engine (\texttt{DockerD}) receives container management requests via its APIs. The engine is in charge of creating container instances and enforcing their specifications via \texttt{containerD} service. 
ContainerD utilizes \texttt{runC} module of the OS kernel to create namespace and cgroups for each container instance.



% \begin{figure}[ht] 
% \begin{subfigure}{0.5\textwidth}
% \includegraphics[width=0.4\textwidth, height=5cm]{Figures/KVMarch.pdf}
% \caption{Modules of KVM hypervisor. Each VM, called Qemu-KVM, has a full-stack of the deployed applications and an operating system. Cgroups is a kernel module of the host that is used to enforce the resource constraints of each VM.}
% \label{fig:KVMarch}
% \end{subfigure}
% \begin{subfigure}{0.5\textwidth}
% \includegraphics[width=0.4\textwidth, height=5cm]{Figures/DockerArch.pdf} 
% \caption{Main modules of Docker. Containers are coupling of \emph{namespace} and \emph{cgroups} modules of the host OS kernel. Docker daemon interacts with Container daemon and runC kernel module to manage containers.}
% \label{fig:DockerArch}
% \end{subfigure}

% \caption{High level architecture of different virtualization platforms}
% \label{fig:image2}
% \end{figure}




% \begin{figure}
%  \centering
%  \includegraphics[width=0.45\textwidth]{Figures/KVMarch.pdf}
%  \caption{Modules of KVM hypervisor. Each VM, called Qemu-KVM, has a full-stack of the deployed applications and an operating system. Cgroups is a kernel module of the host that is used to enforce the resource constraints of each VM.}
%  \label{Fig:KVMarch}
% \end{figure}







%\begin{figure}
%  \centering
%  \includegraphics[width=0.45\textwidth]{Figures/DockerArch.pdf}
%  \caption{Main modules of Docker. Containers are coupling of \emph{namespace} and \emph{cgroups} modules of the host OS kernel. Docker daemon interacts with Container daemon and runC kernel module to manage containers. }
%  \label{Fig:DockerArch}
%   \vspace{-0.2in}
%\end{figure}


\subsection{CPU Provisioning for Virtualized Platforms}\label{subsec:virt}
The host OS generally uses time sharing scheduling policies (\eg Completely Fair Scheduler (CFS) \cite{wong2008fairness}) that does not specify a processing unit (\eg core) to each process. That is, a VM or a container-based process is assigned to a different set of CPU cores of the host machine in each quantum, during their life cycle. In this study, a platform that has its provisioned CPU cores in this default manner is called to be deployed in the \emph{vanilla} mode. 

Alternatively, a user can choose the \emph{pinning} mode, to manually set the CPU cores allocated to a given process (either a VM or a container) and override the default host OS scheduler. We explained the technical details of how to perform CPU pinning in a web-blog post \footnote{How to perform CPU pinning: \url{https://bit.ly/2XrENUM}}. In this case, the host OS scheduler allocates the pinned process only to the specified cores. Note that, unlike vanilla mode that utilizes all the host CPU cores to cumulatively offer the expected performance, for a pinned platform, only the designated cores are utilized and the rest are left idle. As such, the side-effect of pinning (\ie not using the host \os~scheduling) can appear in a lower CPU utilization, hence, it should not be used carelessly for any application. 


%cgroup offers two approaches for assigning CPU cores: 
%\subsubsection{--cpus} logically specifies how many CPU cores should be assigned to a group of processes. For example when a container is started with --cpus=2, cgroup is in charge of limiting the CPU usage of all processes belonging to that container, on all cores and each CPU scheduling cycle. If quantum is defined as the time slice assigned to each process for each CPU scheduling cycle, sum of the CPU usage of all quantum's of a container must be less or equal to the value defined for --cpus where cgroup account and police if required. Default Linux OS scheduler which is CFS (Completely Fair Scheduler) does not bind processes to CPU cores forever,instead, it spawn them differently in each scheduling cycle on various CPU cores, depending of how many cores are available to the OS. As such, it will impose an overhead for cgroup to account for CPU usage of a container if there are numerous CPU cores or many processes are being executed within it.
%\subsubsection{--cpuset-cpus} explicitly specify CPU cores which all processes belonging to this container can utilize. For instant, --cpuset-cpus=0,1,2,3 limits the container to the first four cores of the hardware. Using this method, CFS will just spawn processes on mentioned CPU cores, therefore, it will be much simpler for cgroup to account and police CPU usage, resulting in less overhead. Also, it could be used to assign CPU cores based on some criteria like NUMA to reduce the CPU socket communication and memory sharing overhead. This method is also called \emph{CPU-Pinning} and is valid both for containers and VMs.






% VMM\footnote{Virtual Machine Manager} and performing the resource abstraction and transparency. VMM is in charge of recreating a hardware environment that VM's OS and all applications within it are installed and run. 
%Modern processors are presented by their ISA\footnote{Instruction Set Architecture}, that identify the instruction set used for its modules such as memory, registers as well as its processor. Operating system in addition to any other application that requires to interact with hardware is passing through ISA. While OS directly talk to ISA to access hardware resources using \emph{System ISA}, applications running on the OS utilize \emph{User ISA} that is often called ABI\footnote{Application Binary Interface}. This module handles low-level details for applications to standardize and simplify communication with the hardware.  \emph{Hardware-assisted Virtualization} helps in this regard and Intel provides this feature by Intel-VT, and AMD by AMD-V, which is enabled on almost all CPUs nowadays. %These features are meant to reduce the performance penalties experienced by emulating x86 hardware with hypervisors. 


%\emph{Native Virtual Machine}, sits on top of the hardware and operates as if it is OS, where it can directly interact with hardware through ISA. Hypervisors such as KVM and VMware ESXi are some examples. \emph{Hosted Virtual Machine} are just like an application that requires an OS to run on top of it. As such, when hypervisor wants to interact with hardware, it first pass ABI, then ISA. VMware workstation, OracleVM and Parallels Virtual Machine are using this method. 
%There are mainly two types of hypervisors; \emph{Hosted Virtual Machine} and \emph{Native virtual machines} in which Figure~\ref{Fig:Native-Hostedvm} illustrates with their interaction to ISA and ABI.

%\begin{figure}
%  \centering
%  \includegraphics[width=0.45\textwidth]{Figures/Native-Hostedvm.pdf}
% \caption{Architectural view of two types of hypervisors\cite{BuyyaMasteringBookVirtualizationTaxonomy}}
%  \label{Fig:Native-Hostedvm}
%   \vspace{-0.2in}
%\end{figure}

%\subsubsection{Native virtual machines} Often called 

%OS's running in the VM's will need to interact with their emulated hardware using their own ISA. Since this hypervisors make all hardware resources transparent, many abstraction layers will be added when VM's OS wants to interact with its resources which cause performance penalties. \emph{Para-Virtualization} is used for some resources to lower this overhead. For instance disk or network I/O that are so sensitive to latency requires para-virtualization(\eg VirtIO and SR-IOV storage/net driver in KVM\footnote{Kernel-Based Virtual Machine}, ParaVirtual SCSI storage driver and vmxNet3 network driver in VMware ESXi). 

%\begin{enumerate}
% \item Qemu-KVM creates the machine device emulation code, some mimics real devices and some are special which are called para-virtualized devices. It uses several services from host kernel, the most important one is ioctl() from KVM which is used for guest control. In fact, QEMU is the hypervisor/emulator and KVM is accelerating hypervisor.

% \item Libvirt is to help external services to interact with KVM/QEMU with its APIs. Libvirt is simply a virtualization management library that provides a convenient way to manage VM's and other functions such as disk and nic management. A command line utility called virsh as well as a GUI called virt-manager are some examples that use Libvirt API to manage a KVM hypervisor. In an Openstack deployment, Nova-agent on each KVM host communicates with Libvirt API to control VM's on that compute node.

% KVM has been widely used in industry as it supports advanced features such as hot plug vCPUs, dynamic memory management and Live Migration since February 2007\cite{deepak}. Amazon revealed its developed KVM-based hypervisor called \emph{Nitro} on 2017 where all C5 EC2 instances are using this hypervisor. Many HCIs\footnote{Hyper Converged Infrastructure} are using it as their virtualization platform (\eg Nutanix, Maxta and Cloudistics).
%\end{enumerate}

% There are six namespaces in a Linux OS to the date that determine the specification of a container:
% \begin{enumerate}
% \item{PID} or Process IDs belonging to this container
% %, that partition/aggregate an independent set of PIDs that belong to this namespace. Child processes that these PIDs later generate are aggregated in this namespace as well.
% \item{NET} or Network specification (IP,mask, etc)
% \item{IPC} or Inter Process Communication
% %, isoltates POSIX message queues
% \item{MNT} for storage specification 
% %virtualize a different and isolated view of filesystem’s hierarchy;
% \item{USR}, defines isolated users and groups
% %is to isolate users and groups in addition to their capabilities, permissions and privileges;
% \item{UTS} which isolates hostname
% and NIS (Network Information System) identifiers that are specific for an OS.
% \end{enumerate}
% \\Some benefits of Containers are:
% \begin{itemize}
%     \item Less overhead: Container impose less overhead for virtualization.
%     \item Increased portability: They can be easily cloned with all application within them plus their dependencies, and restored in any architecture, and scalecumulativelyd with automation tools. 
%     \item Better application development: Containers support CI/CD to facilitate ALM\footnote{Application Lifecycle Management}.
% \end{itemize}
%For instance,  Docker is one of the most known lightweight virtualization in cloud environments and is used broadly in industry when manageability and scalability has the highest priority(\eg AWS Serverless Fargate service\cite{ASWFargate}, Azure Container services\cite{AzureContainer}). On the other hand, Singularity is being adopted by many HPC centers\cite{Oleksandr} and is widely used when performance is the primitive requirement(\eg CINECA, PSC, SDSC, NSC).
%Docker was designed for the deployment of microservices in a developer friendly environment whereas CI/CD  as well as integration with automation and orchestration tools such as Kubernetes were essential. By offering these features, Docker could reinvent lightweight virtualization in addition to software developing, shipping, testing, and deploying in production environments.
% \item{Docker Registry} is an application that manages storing and delivery of container images.
% \item{Docker Client} is a command-line interface, communicating with Docker API.
% \item{Libcontainer} is the mastermind behind Docker Engine, in charge of managing container's lifecycle, whether it is image transfer, storage attachment, container execution or supervision (formerly containerd).
% \item{Libnetwork} is managing and controlling inter-communication of containers as well as their communication with the external networks.

==> The Art of CPU-Pinning-OLD/Sources/conclsn.tex <==
\section{Summary and Best Practices}\label{sec:conclsn}

In this study, the performance overhead imposed by different virtualized platforms commonly used in the cloud was studied. Four popular application types, namely video processing and parallel processing (MPI), web processing, and No-SQL were studied. 
The study revealed that: \textbf{(A)} application characteristic (\ie IO-bound versus CPU-bound) is decisive on the imposed overhead of different virtualization platforms. \textbf{(B)} CPU pinning can reduce the overhead of virtualized platforms, particularly for IO-bound applications running on containers. \textbf{(C)} The proportion of container cores to the host cores (we named it CHR) plays a significant role on the overhead of containers. Greater CHR values reduce the overhead. \textbf{(D)} Although containers are known to impose a lower overhead than VMs, the opposite was observed for containers with very low CHRs. \textbf{(E)} Containers on top of VMs (called VMCN) impose a lower overhead for IO intensive applications. \textbf{(F)} Increasing the level of multitasking amplifies the overhead of containers.

In addition, this study provides the following set of \textbf{Best Practices} that can help cloud architects to efficiently configure cloud systems based on their application types:
\begin{shaded*}
\begin{enumerate}
\item Avoid instantiating small vanilla containers (with one or two cores) for any type of application.\vspace{3 mm}
\item For CPU intensive applications (\eg FFmpeg), pinned containers impose the least overhead. \vspace{3 mm}
\item If VMs are being utilized for CPU-bound applications, do not bother pinning them. It neither improves the performance, nor decreases the incurred cost.\vspace{3 mm}
\item For IO intensive applications, if pinned container is not a viable option, then use container within VM (VMCN). It imposes a lower overhead than a VM or a vanilla container.\vspace{3 mm}
\item To minimize the overhead of containers, for CPU intensive applications configure them with $0.07<CHR<0.14$ and for IO intensive applications use $0.14<CHR<0.28$. If the application is ultra IO intensive (\eg Cassandra), even a higher CHR ($0.28<CHR <0.57$) is suggested.

\end{enumerate}
\end{shaded*}
In the further, we plan to extend the study to incorporate the impact of network overhead. In addition, we plan to provide a mathematical model to measure the overhead of a given virtualization platforms based on the isolation level it offers.


==> The Art of CPU-Pinning-OLD/Sources/contingencyrank.tex <==
\begin{table*}[tp]
	\caption{Ranked (R) List of Cyber-Physical Contingencies (MDP edges)}
	\label{tab:cp-contingencies}
	\centering
	\tiny
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} & \textbf{R} & \textbf{Edge} \\ \hline
		0 & $0,74$ & 1 & $0,1$ & 2 & $0,146$ & 3 & $74,125$ & 4 & $74,101$ & 5 & $74,2$ & 6 & $74,134$ & 7 & $74,142$ & 8 & $74,76$ & 9 & $1,2$\\ \hline
		10 & $1,73$ & 11 & $146,142$ & 12 & $146,73$ & 13 & $125,126$ & 14 & $101,123$ & 15 & $101,102$ & 16 & $101,111$ & 17 & $101,119$ & 18 & $101,28$ & 19 & $101,77$\\ \hline
		20 & $2,52$ & 21 & $2,28$ & 22 & $2,3$ & 23 & $2,61$ & 24 & $2,69$ & 25 & $134,139$ & 26 & $134,111$ & 27 & $134,61$ & 28 & $134,135$ & 29 & $134,141$\\ \hline
		30 & $142,145$ & 31 & $142,119$ & 32 & $142,69$ & 33 & $142,143$ & 34 & $142,141$ & 35 & $76,77$ & 36 & $73,69$ & 37 & $126,53$ & 38 & $126,127$ & 39 & $126,103$\\ \hline
		40 & $126,131$ & 41 & $126,133$ & 42 & $123,99$ & 43 & $123,124$ & 44 & $123,118$ & 45 & $123,122$ & 46 & $123,50$ & 47 & $102,103$ & 48 & $111,118$ & 49 & $111,112$\\ \hline
		50 & $111,116$ & 51 & $111,38$ & 52 & $111,87$ & 53 & $119,122$ & 54 & $119,120$ & 55 & $119,46$ & 56 & $119,116$ & 57 & $119,95$ & 58 & $28,50$ & 59 & $28,29$\\ \hline
		60 & $28,38$ & 61 & $28,46$ & 62 & $28,4$ & 63 & $77,99$ & 64 & $77,78$ & 65 & $77,95$ & 66 & $77,4$ & 67 & $77,87$ & 68 & $52,53$ & 69 & $52,75$\\ \hline
		70 & $52,29$ & 71 & $52,66$ & 72 & $52,72$ & 73 & $3,75$ & 74 & $3,4$ & 75 & $3,62$ & 76 & $3,70$ & 77 & $61,66$ & 78 & $61,38$ & 79 & $61,62$\\ \hline
		80 & $61,68$ & 81 & $69,72$ & 82 & $69,46$ & 83 & $69,70$ & 84 & $69,68$ & 85 & $139,131$ & 86 & $139,66$ & 87 & $139,136$ & 88 & $139,112$ & 89 & $139,140$\\ \hline
		90 & $135,136$ & 91 & $135,87$ & 92 & $135,62$ & 93 & $135,138$ & 94 & $141,140$ & 95 & $141,116$ & 96 & $141,68$ & 97 & $141,138$ & 98 & $145,133$ & 99 & $145,72$\\ \hline
		100 & $145,144$ & 101 & $145,120$ & 102 & $145,140$ & 103 & $143,144$ & 104 & $143,95$ & 105 & $143,70$ & 106 & $143,138$ & 107 & $53,54$ & 108 & $53,30$ & 109 & $53,58$\\ \hline
		110 & $53,60$ & 111 & $127,79$ & 112 & $127,54$ & 113 & $127,128$ & 114 & $127,130$ & 115 & $103,79$ & 116 & $103,104$ & 117 & $103,108$ & 118 & $103,30$ & 119 & $103,110$\\ \hline
		120 & $131,58$ & 121 & $131,128$ & 122 & $131,104$ & 123 & $131,132$ & 124 & $133,60$ & 125 & $133,130$ & 126 & $133,108$ & 127 & $133,132$ & 128 & $99,100$ & 129 & $99,94$\\ \hline
		130 & $99,98$ & 131 & $99,26$ & 132 & $124,110$ & 133 & $124,100$ & 134 & $124,115$ & 135 & $124,121$ & 136 & $124,51$ & 137 & $118,94$ & 138 & $118,115$ & 139 & $118,117$\\ \hline
		140 & $118,45$ & 141 & $122,98$ & 142 & $122,121$ & 143 & $122,117$ & 144 & $122,49$ & 145 & $50,26$ & 146 & $50,51$ & 147 & $50,45$ & 148 & $50,49$ & 149 & $112,104$\\ \hline
		150 & $112,115$ & 151 & $112,113$ & 152 & $112,39$ & 153 & $112,88$ & 154 & $116,117$ & 155 & $116,113$ & 156 & $116,43$ & 157 & $116,92$ & 158 & $38,45$ & 159 & $38,39$\\ \hline
		160 & $38,43$ & 161 & $38,14$ & 162 & $87,94$ & 163 & $87,88$ & 164 & $87,14$ & 165 & $87,92$ & 166 & $120,108$ & 167 & $120,121$ & 168 & $120,113$ & 169 & $120,47$\\ \hline
		170 & $120,96$ & 171 & $46,49$ & 172 & $46,47$ & 173 & $46,43$ & 174 & $46,22$ & 175 & $95,98$ & 176 & $95,96$ & 177 & $95,92$ & 178 & $95,22$ & 179 & $29,30$\\ \hline
		180 & $29,51$ & 181 & $29,39$ & 182 & $29,47$ & 183 & $29,5$ & 184 & $4,26$ & 185 & $4,5$ & 186 & $4,22$ & 187 & $4,14$ & 188 & $78,79$ & 189 & $78,100$\\ \hline
		190 & $78,96$ & 191 & $78,5$ & 192 & $78,88$ & 193 & $75,54$ & 194 & $75,5$ & 195 & $75,63$ & 196 & $75,71$ & 197 & $66,58$ & 198 & $66,63$ & 199 & $66,39$\\ \hline
		200 & $66,67$ & 201 & $72,60$ & 202 & $72,71$ & 203 & $72,47$ & 204 & $72,67$ & 205 & $62,63$ & 206 & $62,14$ & 207 & $62,65$ & 208 & $70,71$ & 209 & $70,22$\\ \hline
		210 & $70,65$ & 211 & $68,67$ & 212 & $68,43$ & 213 & $68,65$ & 214 & $136,128$ & 215 & $136,63$ & 216 & $136,88$ & 217 & $136,137$ & 218 & $140,132$ & 219 & $140,137$\\ \hline
		220 & $140,113$ & 221 & $140,67$ & 222 & $138,137$ & 223 & $138,92$ & 224 & $138,65$ & 225 & $144,130$ & 226 & $144,71$ & 227 & $144,96$ & 228 & $144,137$ & 229 & $54,6$\\ \hline
		230 & $54,55$ & 231 & $54,57$ & 232 & $30,6$ & 233 & $30,31$ & 234 & $30,35$ & 235 & $30,37$ & 236 & $58,55$ & 237 & $58,31$ & 238 & $58,59$ & 239 & $60,57$\\ \hline
		240 & $60,35$ & 241 & $60,59$ & 242 & $79,80$ & 243 & $79,84$ & 244 & $79,6$ & 245 & $79,86$ & 246 & $128,55$ & 247 & $128,80$ & 248 & $128,129$ & 249 & $130,57$\\ \hline
		250 & $130,84$ & 251 & $130,129$ & 252 & $104,80$ & 253 & $104,105$ & 254 & $104,31$ & 255 & $104,107$ & 256 & $108,35$ & 257 & $108,84$ & 258 & $108,105$ & 259 & $108,109$\\ \hline
		260 & $110,86$ & 261 & $110,107$ & 262 & $110,109$ & 263 & $110,37$ & 264 & $132,59$ & 265 & $132,129$ & 266 & $132,105$ & 267 & $100,86$ & 268 & $100,91$ & 269 & $100,97$\\ \hline
		270 & $100,27$ & 271 & $94,91$ & 272 & $94,93$ & 273 & $94,21$ & 274 & $98,97$ & 275 & $98,93$ & 276 & $98,25$ & 277 & $26,27$ & 278 & $26,21$ & 279 & $26,25$\\ \hline
		280 & $115,107$ & 281 & $115,114$ & 282 & $115,42$ & 283 & $115,91$ & 284 & $121,109$ & 285 & $121,114$ & 286 & $121,48$ & 287 & $121,97$ & 288 & $51,37$ & 289 & $51,27$\\ \hline
		290 & $51,42$ & 291 & $51,48$ & 292 & $117,93$ & 293 & $117,114$ & 294 & $117,44$ & 295 & $45,21$ & 296 & $45,42$ & 297 & $45,44$ & 298 & $49,25$ & 299 & $49,48$\\ \hline
		300 & $49,44$ & 301 & $113,105$ & 302 & $113,114$ & 303 & $113,40$ & 304 & $113,89$ & 305 & $39,31$ & 306 & $39,42$ & 307 & $39,40$ & 308 & $39,15$ & 309 & $88,80$\\ \hline
		310 & $88,91$ & 311 & $88,15$ & 312 & $88,89$ & 313 & $43,44$ & 314 & $43,40$ & 315 & $43,19$ & 316 & $92,93$ & 317 & $92,89$ & 318 & $92,19$ & 319 & $14,21$\\ \hline
		320 & $14,15$ & 321 & $14,19$ & 322 & $47,35$ & 323 & $47,48$ & 324 & $47,40$ & 325 & $47,23$ & 326 & $96,84$ & 327 & $96,97$ & 328 & $96,23$ & 329 & $96,89$\\ \hline
		330 & $22,25$ & 331 & $22,23$ & 332 & $22,19$ & 333 & $5,6$ & 334 & $5,27$ & 335 & $5,23$ & 336 & $5,15$ & 337 & $63,55$ & 338 & $63,15$ & 339 & $63,64$\\ \hline
		340 & $71,57$ & 341 & $71,23$ & 342 & $71,64$ & 343 & $67,59$ & 344 & $67,40$ & 345 & $67,64$ & 346 & $65,64$ & 347 & $65,19$ & 348 & $137,129$ & 349 & $137,89$\\ \hline
		350 & $137,64$ & 351 & $6,7$ & 352 & $6,11$ & 353 & $6,13$ & 354 & $55,7$ & 355 & $55,56$ & 356 & $57,11$ & 357 & $57,56$ & 358 & $31,7$ & 359 & $31,32$\\ \hline
		360 & $31,34$ & 361 & $35,11$ & 362 & $35,32$ & 363 & $35,36$ & 364 & $37,13$ & 365 & $37,34$ & 366 & $37,36$ & 367 & $59,56$ & 368 & $59,32$ & 369 & $80,81$\\ \hline
		370 & $80,7$ & 371 & $80,83$ & 372 & $84,11$ & 373 & $84,81$ & 374 & $84,85$ & 375 & $86,83$ & 376 & $86,85$ & 377 & $86,13$ & 378 & $129,56$ & 379 & $129,81$\\ \hline
		380 & $105,32$ & 381 & $105,81$ & 382 & $105,106$ & 383 & $107,83$ & 384 & $107,106$ & 385 & $107,34$ & 386 & $109,85$ & 387 & $109,106$ & 388 & $109,36$ & 389 & $91,83$\\ \hline
		390 & $91,18$ & 391 & $91,90$ & 392 & $97,85$ & 393 & $97,24$ & 394 & $97,90$ & 395 & $27,13$ & 396 & $27,18$ & 397 & $27,24$ & 398 & $93,90$ & 399 & $93,20$\\ \hline
		400 & $21,18$ & 401 & $21,20$ & 402 & $25,24$ & 403 & $25,20$ & 404 & $114,106$ & 405 & $114,41$ & 406 & $114,90$ & 407 & $42,34$ & 408 & $42,41$ & 409 & $42,18$\\ \hline
		410 & $48,36$ & 411 & $48,41$ & 412 & $48,24$ & 413 & $44,20$ & 414 & $44,41$ & 415 & $40,32$ & 416 & $40,41$ & 417 & $40,16$ & 418 & $89,81$ & 419 & $89,90$\\ \hline
		420 & $89,16$ & 421 & $15,7$ & 422 & $15,18$ & 423 & $15,16$ & 424 & $19,20$ & 425 & $19,16$ & 426 & $23,11$ & 427 & $23,24$ & 428 & $23,16$ & 429 & $64,56$\\ \hline
		430 & $64,16$ & 431 & $7,8$ & 432 & $7,10$ & 433 & $11,8$ & 434 & $11,12$ & 435 & $13,10$ & 436 & $13,12$ & 437 & $56,8$ & 438 & $32,8$ & 439 & $32,33$\\ \hline
		440 & $34,10$ & 441 & $34,33$ & 442 & $36,12$ & 443 & $36,33$ & 444 & $81,8$ & 445 & $81,82$ & 446 & $83,82$ & 447 & $83,10$ & 448 & $85,82$ & 449 & $85,12$\\ \hline
		450 & $106,82$ & 451 & $106,33$ & 452 & $18,10$ & 453 & $18,17$ & 454 & $90,82$ & 455 & $90,17$ & 456 & $24,12$ & 457 & $24,17$ & 458 & $20,17$ & 459 & $41,33$\\ \hline
		460 & $41,17$ & 461 & $16,8$ & 462 & $16,17$ & 463 & $8,9$ & 464 & $10,9$ & 465 & $12,9$ & 466 & $33,9$ & 467 & $82,9$ & 468 & $17,9$ &   &  \\ \hline
	\end{tabular}
\end{table*}


==> The Art of CPU-Pinning-OLD/Sources/evltn.tex <==
\section{Evaluation}
\label{sec:evaluation}

This is the evaluation part




==> The Art of CPU-Pinning-OLD/Sources/intro.tex <==
\section{Introduction}\label{sec:intro}

%Throughout the last decade, hardware virtualization impressively enhanced compute agility, utilization, consolidation, reliability and manageability. Taking advantage of these features, cloud data centers appeared which completely changed the usage model of IT infrastructures from purchasing everything and operating the infrastructure with a very complex IT operation organizational chart to renting it as a service from a service provider with a much more simpler operation staff organizational chart. With that said, outsourcing IT infrastructure with IaaS\footnote{Infrastructure as a Service} service, helped companies and institutes to get rid of many problems involved in CapEx\footnote{Capital Expenditure} and OpEx\footnote{Operational Expenditure} of a data center from hardware perspective\cite{BuyyaPrincipleBook-OpexCapex, Gautam-OpexCapes}, however, performance overhead resulting from many abstraction layers in the hypervisor\cite{ZhengLi,Morabito,Felter,Barik} is an obvious disadvantage that is attached to the virtualization technology which is widely used in IaaS. Furthermore, yet the Operating System needs to be managed by customers themselves, therefore they will be still engaged with OpEx. Answering the question of “is there any way to offload OS\footnote{Operating System} operation tasks as well to the cloud provider and just concentrate on the application itself” is server-less computing where container technology is enabler for this emerging cloud service\cite{Barik,Lloyd,Rajan}.  

%Designed as light-weighted as possible, made containers the perfect virtualization technology on top of which to build the server-less computing that we see it in cloud providers service portfolio nowadays(\eg AWS Lambda\cite{ASWLambda}, Azure Service Fabric\cite{AzureFabric}). Less virtualization overhead, storage footprint and provisioning time, enhanced scalability, application packaging and portability as well as complete CI/CD\footnote{Continues Integration/Continues Delivery} and automation tools integrity are some impressive unique features of containers. In contrast to its advantages, security concerns for sharing the kernel of the OS, considerable networking overhead as well as less flexibility for the OS options are some caveats that need to be taken care off when there is a dilemma about application of this technology\cite{Fridriksson,Oleksandr}. These two virtualization technologies are not against each other, and could be mixed to leverage both technologies advantages. It is common to use VMs (Virtual Machines) for running applications\cite{Ilias}, although, having yet another software layer for handling containers that are wasting precious resources is questionable if performance is a vital requirement.  
Hardware virtualization in form of virtual machines (VMs) is an indispensable part of cloud computing technology that offers isolation, manageability, consolidation, and reliability~\cite{parashar2013cloud} to cloud-based applications. However, performance overhead, resulted from several abstraction layers in the hypervisor~\cite{ZhengLi,Morabito,felter2015updated,Barik}, has historically been a side-effect of the virtualization technology. More recently, a lightweight virtualization technology, known as containerization, that provides abstraction at the application layer has gained popularity in the cloud era. Numerous cloud services, such as serverless computing~\cite{peekserverless,lloyd2018serverless} (\eg AWS Lambda~\cite{ASWLambda}, Azure Service Fabric\cite{AzureFabric}), are offered based on containers. However, we note that containerization is even making a deeper shift in application deployment, such as those used to manage critical layers of IT infrastructure. For instance, containers are being utilized in storage appliances (\eg EMC Unity~\cite{EMCUnity}) to reduce the fail-over time and improve their availability. In addition to negligible imposed overhead, containers are more storage-efficient, have shorter cloning and application deployment time, faster scale out, and offer Continuous Integration/Continuous Delivery (CI/CD)~\cite{nogueira2018improving}. Nonetheless, conflicts between processes sharing the kernel and lack of cross middleware portability are known drawbacks of the containerization~\cite{dupont2017edge}.


The pros and cons of each virtualization technology in addition to the possibility of deploying an application on bare-metal (\eg Dedicated EC2 instances in AWS) has offered cloud solution architects a range of \emph{execution platforms} (\ie bare-metal, VMs, containers, and containers on top of VMs) to deploy a certain application on the cloud. 
In particular, each application has its own characteristics that can reap the benefits of a certain type of execution platform and undergoes a different overhead. For instance, database servers are known to take advantage of bare-metal platforms, due to high volume of disk operations~\cite{zhang2012distributed}, whereas web servers benefit from \emph{virtualized platforms} (\ie VMs, containers, and containers within VMs) that offer a higher portability~\cite{yu2015live,qiu2017lxc,dupont2017edge}. 

It is challenging for a cloud solution architect to efficiently deploy a certain application via choosing a proper execution platform. In a multi-tier application, this can potentially lead to choosing distinct execution platforms for deployment of each application tier~\cite{bi2017application}. The challenge becomes further complicated when we know that the overhead of each execution platform can remarkably vary, depending on the way the execution platform is configured on the underlying hardware resources. Specifically, CPU provisioning for virtualized platforms can be configured either through CPU-quota or CPU-set (a.k.a \emph{CPU pinning})~\cite{podzimek2015analyzing}. In the former, at each scheduling event, the middleware of the host machine decides about allocating the proper CPU core(s) to each VM/container, whereas, in the latter, certain CPU cores are statically bound to each VM/container by the solution architect. Our hypothesis is that CPU pinning can drastically reduce the overhead of virtualized platforms. However, it is noteworthy that extensive CPU pinning incurs a higher cost and makes the host management more challenging. 

%In this panorama, bench-marking is a great help to survey and analyze each virtualization technology overhead for some kind of workloads that reflects day-to-day use case of applications. Certainly, similar evaluations have been performed in recent years but as these technologies are no exception of software development cycles and update procedures, bench-marks need to be updated as well. As such, performance evaluation is not a one time for all the times task, and it should be recurring. 
%What is found while the process of bench-marking in this work is when working with VMs and containers, the way computing resources are assigned matters to the OS scheduler and modules that are in charge of making resource boundaries for VMs or Containers. With not properly provisioned resources, we can get worst performance overhead specially in the case of containers.

%%%%%%%%%%%%%%%%%%%%% Figure from background, place here to show next page
\begin{figure*}[b!] 
\vspace{-5px}
\centering
\subfloat[ Modules of KVM hypervisor. Each VM, called Qemu-KVM, has a full-stack of the deployed applications and an operating system. Libvirt provides necessary APIs for managing KVM.]{
{
\includegraphics[width=0.38\textwidth]{Figures/KVMarch.pdf}}
\label{fig:KVMarch}
}
\hspace{5pt}
\subfloat[Main modules of Docker. Containers are coupling of \texttt{namespace} and \texttt{cgroups} modules of the host OS kernel. Docker daemon interacts with Container daemon (\texttt{ContainerD}) and \texttt{runC} kernel module to manage containers.]{
{
\includegraphics[width=0.38\textwidth]{Figures/DockerArch.pdf} 
\label{fig:DockerArch}
}
}
%\vspace{-6px}
\caption{High level architecture of different virtualization platforms.}
\label{fig:image2}
\end{figure*}


The \emph{goal} of this study is to unveil the imposed overhead of each virtualization platform for different application types commonly deployed on the cloud. Further, we study the impact of various CPU provisioning configurations for the underlying hardware resources. 

To achieve the goal, we conduct an extensive performance evaluation on the following four application types that exhibit different processing characteristics and are commonly used in the cloud: (A) \emph{FFmpeg}~\cite{ffmpeg16} is a video transcoding application that exhibits a CPU-bound behavior; (B) \emph{MPI}~\cite{gropp1999using} applications that represent parallel processing behavior; (C) \emph{WordPress}~\cite{patel2011performance} is a web-based system representing many short tasks with IO-bound behavior; (D) \emph{Apache Cassandra}~\cite{abramova2013nosql} is a NoSQL database management system representing an extensive IO-bound behavior within a single large process.

Each application type is deployed under various resource configurations (a.k.a instance type) on our private cloud. Specifically, we evaluate the imposed overhead of different execution platforms using different number of CPU cores and under two circumstances---when CPU pinning is in place and when it is not. In summary, the \emph{contributions} of this paper are as follows:
\begin{itemize}
  \item Measuring and analyzing the imposed overhead of different execution platforms for widely-used cloud-based applications.
  \item Analyzing the impact of altering resource configurations, including number of CPU cores and CPU pinning, on the imposed overhead of different execution platforms.
  \item Proposing a set of best practices for deploying different application types in different virtualization platforms.
\end{itemize}

%The \emph{outcomes} of this study is twofold: (A) It offers solution architects best practices in deploying a given application on the cloud; and (B) It assists IaaS cloud service providers to enforce efficient allocation policies to arriving VM/container requests, such that the unnecessary overhead of virtualization is avoided. 

This paper is structured as follows. Section \ref{sec:background} provides an architectural view of virtualization platforms and describes CPU provisioning models. Section \ref{sec:PerfStudyanalysis} describes the applications, our testbed, and analyzes the overhead of different platforms under various configurations. In Section \ref{sec:cross}, we perform a cross-application overhead analysis of the imposed overhead across different application types. Section \ref{sec:relwk} presents the most relevant works in the literature for benchmarking virtualization platforms and the use of pinning. Then, in Section \ref{sec:conclsn}, we summarize the lessons learnt and provide a set of best practices to efficiently configure cloud platforms.

==> The Art of CPU-Pinning-OLD/Sources/mdptable.tex <==
\begin{table*}[tp]
	\caption{Mappings between MDP State IDs (Figure \ref{fig:agt}) and Compromised Asset IDs}
	\label{tab:ip-host}
	\centering
	\tiny
	\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
		\hline
		\textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} & \textbf{State} & \textbf{Assets} \\ \hline
		0 & 6 & 1 & 61 & 2 & 610 & 3 & 6102 & 4 & 61023 & 5 & 610234 & 6 & 6102349 & 7 & 61023495 & 8 & 610234957\\ \hline
		9 & 6102349578 & 10 & 610234958 & 11 & 61023497 & 12 & 610234978 & 13 & 61023498 & 14 & 610235 & 15 & 6102354 & 16 & 61023547 & 17 & 610235478\\ \hline
		18 & 61023548 & 19 & 6102357 & 20 & 61023578 & 21 & 6102358 & 22 & 610237 & 23 & 6102374 & 24 & 61023748 & 25 & 6102378 & 26 & 610238\\ \hline
		27 & 6102384 & 28 & 6103 & 29 & 61034 & 30 & 610349 & 31 & 6103495 & 32 & 61034957 & 33 & 610349578 & 34 & 61034958 & 35 & 6103497\\ \hline
		36 & 61034978 & 37 & 6103498 & 38 & 61035 & 39 & 610354 & 40 & 6103547 & 41 & 61035478 & 42 & 6103548 & 43 & 610357 & 44 & 6103578\\ \hline
		45 & 610358 & 46 & 61037 & 47 & 610374 & 48 & 6103748 & 49 & 610378 & 50 & 61038 & 51 & 610384 & 52 & 6104 & 53 & 61049\\ \hline
		54 & 610492 & 55 & 6104925 & 56 & 61049257 & 57 & 6104927 & 58 & 610495 & 59 & 6104957 & 60 & 610497 & 61 & 6105 & 62 & 61052\\ \hline
		63 & 610524 & 64 & 6105247 & 65 & 610527 & 66 & 61054 & 67 & 610547 & 68 & 61057 & 69 & 6107 & 70 & 61072 & 71 & 610724\\ \hline
		72 & 61074 & 73 & 617 & 74 & 60 & 75 & 61024 & 76 & 602 & 77 & 6023 & 78 & 60234 & 79 & 602349 & 80 & 6023495\\ \hline
		81 & 60234957 & 82 & 602349578 & 83 & 60234958 & 84 & 6023497 & 85 & 60234978 & 86 & 6023498 & 87 & 60235 & 88 & 602354 & 89 & 6023547\\ \hline
		90 & 60235478 & 91 & 6023548 & 92 & 602357 & 93 & 6023578 & 94 & 602358 & 95 & 60237 & 96 & 602374 & 97 & 6023748 & 98 & 602378\\ \hline
		99 & 60238 & 100 & 602384 & 101 & 603 & 102 & 6034 & 103 & 60349 & 104 & 603495 & 105 & 6034957 & 106 & 60349578 & 107 & 6034958\\ \hline
		108 & 603497 & 109 & 6034978 & 110 & 603498 & 111 & 6035 & 112 & 60354 & 113 & 603547 & 114 & 6035478 & 115 & 603548 & 116 & 60357\\ \hline
		117 & 603578 & 118 & 60358 & 119 & 6037 & 120 & 60374 & 121 & 603748 & 122 & 60378 & 123 & 6038 & 124 & 60384 & 125 & 604\\ \hline
		126 & 6049 & 127 & 60492 & 128 & 604925 & 129 & 6049257 & 130 & 604927 & 131 & 60495 & 132 & 604957 & 133 & 60497 & 134 & 605\\ \hline
		135 & 6052 & 136 & 60524 & 137 & 605247 & 138 & 60527 & 139 & 6054 & 140 & 60547 & 141 & 6057 & 142 & 607 & 143 & 6072\\ \hline
		144 & 60724 & 145 & 6074 & 146 & 67 &   &   &   &   &   &   &   &   &   &   &   &  \\ \hline
	\end{tabular}
\end{table*}


==> The Art of CPU-Pinning-OLD/Sources/rw.tex <==
\section{Related Work}\label{sec:relwk}
Container technology has gained a major attention over the past few years, thus, several research works have been undertaken to evaluate their performance in contrast to VMs. Xavier \etal~\cite{xavier2013performance} compared the Linux VServer, OpenVZ, and Linux Containers (LXC) with Xen hypervisor using synthetic workloads such as LINPACK, STREAM and IOzone. They observed that containers can provide a near-native performance for the mentioned workloads. However, this work does not consider popular cloud applications and platforms. In another study, Shirinbab \etal~\cite{shirinbab2017performance} compare the performance of Docker, VMware ESXi, and Bare-Metal. They evaluated the performance of these platforms for Apache Cassandra database. Their work shows that in terms of disk I/O, containers incur a performance penalty, specially for disk write operations.

In \cite{saha2018evaluation}, authors evaluated the network overhead of Docker and Singularity containers using HPCG and miniFE workloads. Rudyy \etal~\cite{rudyy2019containers} also compared three different container technologies on computational fluid dynamics (CFD) and concluded Singularity is the suitable container solution for HPC workloads that provide the same execution time as Bare-Metal. Mavridis and Karatza~\cite{mavridis2017performance} studied containers on VMs configuration. Similar to \cite{xavier2013performance}, they evaluated Docker on top of KVM VMs using well-known benchmarking tools and explored the overhead in comparison with Bare-Metal. They concluded adding another virtualization layer that helps for easier management and system maintenance, but incurs a performance cost.

Several research works compared containers versus VMs and Bare-Metal \cite{xavier2013performance,shirinbab2017performance,saha2018evaluation,rudyy2019containers,ZhengLi, Morabito,felter2015updated,Barik}. Only few of these studies explored VMCN configuration, which is a popular platform in the cloud \cite{mavridis2017performance}. In addition, majority of the comparisons are performed using synthetic workloads and benchmarking tools such as LINPACK, STREAM, and NetPerf that exhibit different  behavior than real cloud-based workloads.

% In our research, by utilizing aforementioned works, we 
% \begin{itemize}
%     \item study more on the performance overhead of containers on top of VMs, and compare it to VMs, Bare-Metal an also containers on top of Bare-Metal.
%     \item choose three different kinds of applications for the workload, which are used in industry; FFmpeg for video processing, MPI as HPC case and a WordPress website as a popular use-case of containers in cloud data centers.
%     \item included variety in resources of containers to explore the trend of the overhead when the number of CPU cores increase and impact of CPU-pinning
% \end{itemize}

==> The Art of CPU-Pinning-OLD/Sources/sec-apndx.tex <==
\section{Appendix}\label{sec:apndx}

\begin{lemma}
\label{LeftCosetsDisjoint}
Let $N$, $C(k)$, and $S(k)$ be the total number of network nodes, compromised set of nodes, and secure (non-compromised) network nodes, respectively. Also, we define $V$ and $\beta(k)$ to be, respectively, the vulnerability factor, and the number of network nodes which get compromised at the $k$-th step during the MDP generation phase. 
Then
\begin{equation}
\beta(k+1) = N\cdot\big(\frac{N-V}{N}\big)^{\frac{\log(1-\frac{C(k)}{N})}{\log(\frac{N-V}{N})}}\cdot\Big[ 1 - \big(\frac{N-V}{N}\big)^{\beta(k)} \Big],
\end{equation}

\end{lemma}

\begin{IEEEproof}
Clearly, the number of internal compromised network nodes is initially zero, i.e., $C(0) = 0$. Given the vulnerability factor of $V$, the next step of the MDP generation will result in $C(1) = V$, i.e., $V$ new MDP states. Next, \name will use each of the $V$ compromised nodes, and the non-compromised hosts which are accessible from any of those $V$ compromised nodes, to further expand the MDP model. It is important to mention that exploration of every compromised node will result in $\leq V$ new compromised nodes as some them may have already been compromised during one of the previous steps. 

We calculate the expected number of non-compromised network nodes which are visited (get compromised) at the $k$-th step of the MDP generation procedure, i.e., $\beta(k+1)$. Clearly, those network nodes are visited through investigation of the nodes which got newly compromised during the previous phase $\beta(k)$. Once the first node out of the $\beta(k)$ nodes is investigated, the expected number of compromised nodes is $E[c_k(1)] = C(k) + V\cdot\frac{N-C(k)}{N}$, where $V\cdot\frac{N-V}{N}$ new nodes are compromised, because $V$ (vulnerability factor) nodes are selected which are each non-compromised with probability $\frac{N-V}{N}$. Following some algebraic calculations and arrangements, we have the closed form solution 
\begin{equation}
c_0(n) = N\cdot\Big[1-\big(\frac{N-V}{N}\big)^{n}\Big],
\end{equation}
and hence, we calculate $\beta(k+1)$ as $C(k+1) - C(k)$:
\begin{equation}
\beta(k+1) = N\cdot\big(\frac{N-V}{N}\big)^\alpha\cdot\Big[ 1 - \big(\frac{N-V}{N}\big)^{\beta(k)} \Big],
\end{equation}
where
\begin{equation}
\alpha = \frac{\log(1-\frac{C(k)}{N})}{\log(\frac{N-V}{N})}.
\end{equation}

\qed
\end{IEEEproof}

==> The Art of CPU-Pinning-OLD/Sources/sec-index.tex <==

\section{Cyber-physical Security Index}\label{sec:index}

\name uses a new power grid security index to evaluate the security level of each MDP state. The proposed index takes into consideration the severity of the potential malicious physical consequences (i.e. percentage of line overload) and the difficulty to penetrate into the power network. In particular, using a defense-centric metric, \name measures how susceptible the power system is to cyber attack induced contingencies, e.g., line outages, at every MDP state. As explained in the previous section, states capture the set of contingencies that can occur due to malicious actions. Then, \name makes use of an adversary-driven metric to quantify how the attackers can obtain the required privileges to cause those physical contingencies.  Note that the physical contingencies considered here are steady-state contingencies.  Although not discussed, \name could potentially be modified to study transient contingencies as well.

Here, to measure the power system's susceptibility to cyber attack induced contingencies (e.g., line outages) for each state, \name updates the admittance matrix according to the line outages encoded in that state, and solves the AC power flow equations using the iterative Newton-Raphson algorithm to calculate the line flows. Alternatively, an approximate DC model may be used, requiring only a linear solution, but potentially sacrificing detail \cite{dcpowerflowrevisited}.  
% Saman: In traditional power system contingency Analysis, the impacts of contingencies on an electric power system are quantified and finally prioritized.
\name estimates the susceptibility degree using a modified version of the performance index \cite{davis:multipleoutage} that assigns $0$ to a state if there are no line flow violations and a positive value otherwise, computed using the following equation:
\begin{equation}
F(s) =  \sum_{l \in L}  \big[ \max\{\frac{f_s(l)}{f^{MAX}(l)}-1,0 \} \big] ^2.
\end{equation}
Here, $L$ is the set of all lines, $f_s(l)$ denotes flow on line $l$ in state $s$, and $f^{MAX}(l)$ denotes the maximum flow allowed on line $l$.  In the event that a power flow fails to converge, a severe physical impact can be assumed which justifies setting $F(s)$ to a large number, the outage severity.  The outage severity should be much larger than any of the line severity measures.

To calculate the overall cyber-physical security index for each state $I: s \rightarrow \mathbb{R}$, \name uses the above power system performance index in the following dynamic programming equation:
\begin{equation}\label{eq:dynprog}
% I(s) = \max_{a \in A(s)} \{ F(s) + \gamma\cdot\sum_{s' \in S} [P(s'|s,a).I(s')] \},
I(s) = \max_{a \in A(s)} \{\gamma\cdot\sum_{s' \in S} P(s'|s,a)[\Delta F(s,s') + I(s')] \},
\end{equation}
where $I(.)$ (as the MDP's value function) is formulated as a function of difficulty levels of various cyber attack paths $P(s'|s,a)$ and their physical impact $\Delta F(s,s') = F(s') - F(s)$. To solve Equation \eqref{eq:dynprog}, \name implements the value iteration algorithm.  As formulated, proximity of the attacker to a physical component, existence of easy-to-traverse attack paths, and high final physical impacts of the attacks improve the fitness of a system state from the point of view of the adversary.


==> The Art of CPU-Pinning-OLD/Sources/sec-ovrvw.tex <==
\section{Overview}\label{sec-ovrvw}

\begin{figure*}[tp]
  \centering
  \includegraphics[width=0.95\textwidth]{./Figures/Architecture-crop}
  \caption{High-level Architecture of the \name Framework}
  \label{fig:arch}
\end{figure*}

